Routing in an Uncertain World: Adaptivity, Efficiency, and Equilibrium

We consider the traffic assignment problem in nonatomic routing games where the players' cost functions may be subject to random fluctuations (e.g., weather disturbances, perturbations in the underlying network, etc.). We tackle this problem from the viewpoint of a control interface that makes routing recommendations based solely on observed costs and without any further knowledge of the system's governing dynamics -- such as the network's cost functions, the distribution of any random events affecting the network, etc. In this online setting, learning methods based on the popular exponential weights algorithm converge to equilibrium at an $\mathcal{O}({1/\sqrt{T}})$ rate: this rate is known to be order-optimal in stochastic networks, but it is otherwise suboptimal in static networks. In the latter case, it is possible to achieve an $\mathcal{O}({1/T^{2}})$ equilibrium convergence rate via the use of finely tuned accelerated algorithms; on the other hand, these accelerated algorithms fail to converge altogether in the presence of persistent randomness, so it is not clear how to achieve the "best of both worlds" in terms of convergence speed. Our paper seeks to fill this gap by proposing an adaptive routing algortihm with the following desirable properties: $(i)$ it seamlessly interpolates between the $\mathcal{O}({1/T^{2}})$ and $\mathcal{O}({1/\sqrt{T}})$ rates for static and stochastic environments respectively; $(ii)$ its convergence speed is polylogarithmic in the number of paths in the network; ${(iii)}$ the method's per-iteration complexity and memory requirements are both linear in the number of nodes and edges in the network; and ${(iv)}$ it does not require any prior knowledge of the problem's parameters.

==> AcceleWeight.tex <==
%----------------------------------------------------------------------
%%% ACCELEWEIGHT
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


We now turn our attention towards the stationary regime: in every epoch, we consider a fixed game instance $\game_{\sample}$ (where $\sample$ remains unknown) and observe the precise congestion costs of implemented flows (as considered in Example~\ref{exam:stationary}). Note again that in this case, the mean game $\mgame$ coincides with~$\game_\sample$.

%%% In this setting, note that the mean game is the same as the (fixed) game instance considered in each epoch and that $\cost(\flow) = \costalt (\flow, \rat)$ and $\frac{\partial \cost}{\partial \flow_{\pair, \route}} (\flow) = \rat_{\pair} \sum_{\edge \in \route} \late_{\edge} \parens*{\sum_{\pair \in \pairs} \rat_{\pair} \flow_{\edge}} = \rat_{\pair} \sum_{\edge \in \route} \late_{\edge} (\flow, \rat)$.
%where the learner has full information over the observed costs.


In this context, it is reasonable to expect that a faster convergence rate should be attainable than what provided by the \ac{EW} template: since the equilibrium flows are solutions of a convex minimization problem, a natural question is whether the iconic $\bigoh(1/\nRuns^{2})$ convergence rate of Nesterov is achievable in our case.
% %%% More precisely, it is known that under Lipschitz continuity the rate of $\bigoh(1/\sqrt{\nRuns})$ is unimprovable. That said, whenever smoothness kicks in the iconic rate of $\bigoh(1/\nRuns^{2})$ is achievable by applying Nesterov's acceleration schemes. To that end, taking a more detailed look on the problem's specifics, one can show that the latter is actually the case.
To that end, taking a more detailed look on the problem's specifics at hand, we show that this is actually the case for \eqref{OPT1} (when $\sample$ does not vary). The key enabling fact for this is the following proposition regarding the smoothness level of $\cost$ (its proof is presented in Appendix~\ref{app:acceleweight}):\footnote{Recall that $\length$ is the length of the longest path in $\routes$ and $\lips$ is the Lipschitz constant of $\late_\edge(\cdot, \sample), \forall \edge \in \edges$.}
%
\begin{proposition}\label{propo:potential}
    Suppose that Assumption~\ref{assum:blanket} holds, then $\cost$ is a $\smooth$-smooth convex function over $\flows$ \wrt the $\norm{\cdot}_1$ norm where \mbox{$\smooth:=\length \bderiv$}.
\end{proposition}    
 
%
%
% This proposition raises two key-points: $(i)$ the convergence rate $\bigoh \parens{1/\nRuns^{2}}$ is achievable, \eg by applying Nesterov's acceleration and $(ii)$ classical EW,  while having an (almost) dimension-free property, is sub-optimal for the deterministic landscape since it only ensures at most $\bigoh\parens*{1/\nRuns}$ under smoothness condition.
% %\footnote{See \eg \cite{BBT17} and references therein.}
%
By this token, the rest of this section is devoted to merging the Nesterov's acceleration techniques into the EW template in order to achieve the best of both worlds: the proposed algorithm \textendash\ dubbed \ac{AcceEW} \textendash\ achieves an $\bigoh(\log(\nRoutes) / \nRuns^{2})$ convergence rate which is optimal both in $\nRuns$ and the dependence on the dimensionality of the problem (reflected here on the number of paths $\nRoutes$ over which traffic is routed). The algorithm is presented in pseudo-code form below, and our main theoretical guarantee is provided in Theorem~\ref{theo:acceleweight}.
% %: can we combine these two techniques to achieve the eminence from both ends? We answer this question positively: we analyze an accelerated version of EW---which we term \ac{AcceEW}---that meets these desired features. A pseudo-code of \ac{AcceEW} is given in Algorithm~\ref{algo:AdaExpGrad} and its convergence property is presented via Proposition~\ref{propo:AccExpoGrad}. 

% % Note that in the deterministic setting, the observed congestion cost in the query at Line~\ref{line:AcceEW_dpoint} is the actual cost, \ie $\late_{\edge} \parens*{\ppointalt^{\run-1},\rat} = \late_{\edge} \parens*{\flow^{\rat}_{\edge}}$. 





% % Now,  having all this at hand our candidate iterative solution scheme should combine the best of of both worlds,\ie


% % In terms of performance, \ac{AcceEW} achieves an optimal\footnote{We can construct a routing game instance guaranteeing that any algorithm yields a convergence rate that is lower-bounded by $\Theta\parens*{\nRuns^{-2}}$ based on similar results of \cite{nemirovski2004prox} for convex~optimization.} speed of convergence of order $\bigoh \parens*{\log\parens{\nRoutes} / \nRuns^{2}}$ which of course outperforms the EW Algorithm; alternatively, it only takes at least an $\bigoh \parens*{\eps^{-1/2}}$ number of iterations of \ac{AcceEW} to obtain an $\eps$-approximate solution of \eqref{OPT1}. Moreover, its convergence rate still maintains the same logarithmic order in terms of $\nRoutes$ as that of the EW Algorithm; this shows the scalability of the \ac{AcceEW} Algorithm since in practice, it is often the case that $\nRoutes$ is exponentially large.
% % Formally, this is stated by the following proposition (for a detailed proof we refer the reader to \ref{sec:appen_acceEW}).


% %In this section, we focus on the deterministic setting and look for an algorithm providing better convergences guarantee than that of the EW Algorithm. 

% %The drawbacks of the EW Algorithm analyzed in the previous section comes from the fact that it relies on the Lipschitz-continuity of the function $\cost$ while under Assumptions~\ref{assum:rate} and~\ref{assum:latency}, one might obtain an even stronger property of $\cost$. Particularly, let us denote $\length$ the length of longest paths in $\graph$, we obtain the following~proposition (see \ref{sec:appen_smooth_proof} for a~proof):
% %
% %\begin{proposition}\label{propo:potential}
%     %In any routing game under Assumptions~\ref{assum:rate} and~\ref{assum:latency}, the corresponding function $\cost$ defined in \eqref{eq:RosenthalPhi} is a $\smooth$-smooth convex function over $\flows$ \wrt the $\norm{\cdot}_1$ norm; here, \mbox{$\smooth:= \ratmax^2 \length \bderiv$}.
% %\end{proposition}    
%


\begin{algorithm}[h!]
    \SetKw{Return}{Return} %Change keyword return to Return
	\KwIn{Parameter $\smooth$}
			%%%%%%%%%%%%%%
		 Initialize $\dpoint^{\beforestart}= \boldsymbol{0} \in \R^{\nRoutes}$, $\step^{\beforestart} = 0$ and $\stepalt^{\beforestart}= \frac{1}{\nPairs \massmax \smooth} $ \label{line:AcceEW_initial} \;
		 %
			%
		\For{\run = \start, \afterstart, \ldots}{ 
		     %
		     $\ppoint^{\run} \!=\! \logit (\dpoint^{\run-1})$\;\label{line:AcceEW_ppoint}
    			 %
			$\flow^{\run} = \step^{\run-1} \flow^{\run-1} + (1 - \step^{\run-1}) \ppoint^{\run}$  \; \label{line:AcceEW_flow}%
			%
			 $\stepalt^{\run} = \frac{1}{2} \bracks*{ {2\stepalt^{\run-1} +\stepalt^{\beforestart}}   +     \sqrt{ 4 \stepalt^{\run-1} \stepalt^{\beforestart} + (\stepalt^{\beforestart})^2   } }$\;\label{line:AcceEW_stepalt}
			%
			 $\step^{\run} = {\stepalt^{\run-1}} \big/ {\stepalt^{\run}} $\;\label{line:AcceEW_step}
			%
			 $\ppointalt^{\run} = \step^{\run} \flow^{\run} + (1 - \step^{\run} ) \ppoint^{\run}$\;\label{line:AcceEW_dpoint}
		     %
		     $\dpoint^{\run} \!=\! \dpoint^{\run-1} \!-\! \parens{1 \!-\! \step^{\run}} \stepalt^{\run} \Late \parens*{\ppointalt^{\run},\sample} $\;
		     %
			}	
    \caption{\acl{AcceEW}} \label{algo:AccExpGrad}
\end{algorithm}
%

% Formally, this is stated by the following proposition .



% \begin{algorithm}[h!]
%     \SetKw{Return}{Return} %Change keyword return to Return
% 	\KwIn{Parameter $\smooth$}
% 			%%%%%%%%%%%%%%
% 		 Initialize $\dpoint^{\beforestart} \in [0,1]^{\nRoutes}$ where $\dpoint^{\beforestart}=0$, $\forall \pair \in \pairs$, $\forall \route \in \routes_\pair$\;
% 		 %
% 	    Initialize $\step^{\start} = 0, \stepalt^{\start}= \frac{1}{\nPairs \smooth} $ \;
% 			%
% 		\For{\run = \start, \afterstart, \ldots}{ 
% 		     %
% 		    %
% 		     $\ppoint^{\run}_{\pair, \route} \!=\! \frac{\exp \parens*{\dpoint^{\run-1}_{\pair, \route}} }{ \sum \limits_{\routealt \in \routes_\pair} \exp \parens*{ \dpoint^{\run-1}_{\pair, \route}} } $, $\forall \pair \in \pairs$, $\forall \route \in \routes_\pair$\; \label{line:AcceEW_ppoint}
%     			 %
% 			\Return{$\flow^{\run} = \step^{\run} \flow^{\run} + (1 - \step^{\run}) \ppoint^{\run}$}\; \label{line:AcceEW_flow}%
% 			%
% 			 $\stepalt^{\run+1} = \frac{ \parens*{2\stepalt^{\run} + \frac{1}{  \nPairs \smooth}}   +     \sqrt{ \parens*{\parens{2\stepalt^{\run} + \frac{1}{\nPairs \smooth}}}^2 - 4 \parens{\stepalt^{\run}} ^2 } }{2}$\;\label{line:AcceEW_stepalt}
% 			%
% 			 $\step^{\run+1} = \frac{\stepalt^{\run}}{\stepalt^{\run+1}} $\;\label{line:AcceEW_step}
% 			%
% 			 $\ppointalt^{\run} = \step^{\run+1} \flow^{\run} + (1 - \step^{\run+1} ) \ppoint^{\run}$\;\label{line:AcceEW_dpoint}
% 		     %
% 		     $\dpoint^{\run} = \dpoint^{\run-1} - \parens{1- \step^{\run+1}} \stepalt^{\run+1} \nabla \cost \parens*{\ppointalt^{\run}} $\;
% 		     %
% 			}	
%     \caption{\acl{AcceEW}} \label{algo:AccExpGrad}
% \end{algorithm}

%In the convex optimization literature, there exist the class of accelerated gradient descent algorithms that makes use of the smooth-continuity of the objective function to obtain a better convergence rate than that of the EW Algorithm. Inspired by this, we propose a novel algorithm for the equilibrium-learning problem of the routing game, called the \acl{AcceEW} (\ac{AcceEW}) Algorithm; its pseudo-code is given in Algorithm~\ref{algo:AccExpGrad}. We obtain the following~proposition regarding the convergence properties of \ac{AcceEW} Algorithm:
%
%
\begin{restatable}{theorem}{AccExpoGradPropo} \label{theo:acceleweight}
Suppose that Assumption~\ref{assum:blanket} holds and Algorithm~\ref{algo:AccExpGrad} is run for $\nRuns$ epochs with $\smooth$ defined as in Proposition~\ref{propo:potential}.
Then, in the \emph{stationary regime}, 
the traffic flow profile $\flow^{\nRuns}$ enjoys the following convergence rate:
%computed at any iteration $\run$, $\flow^{\run} \in \flows$; moreover, for any equilibrium normalized flow $\flowbase \in \flows$, in the stationary regime, we have
%
\begin{equation}
\cost\parens*{\flow^\nRuns} - \cost\parens*{\flowbase} \le \frac{4 \nPairs \masssum  \massmax \smooth \log\parens*{\frac{\nRoutes \massmax^2}{\masssum}}  }{\parens*{\nRuns-\start}^2} = \bigoh \parens*{ \frac{\log(\nRoutes)}{\nRuns^2}}, \label{eq:theo_acceleweight}
\end{equation}
where $\flowbase\in\flows$ is any mean equilibrium flow of $\game$.
\end{restatable}
%

%
We give a proof of Theorem~\ref{theo:acceleweight} in Appendix~\ref{app:acceleweight} with an explicit convergence rate in terms of other primitive parameters of the games.  Importantly, Theorem~\ref{propo:AccExpoGrad} confirms that \ac{AcceEW} learns the equilibrium flows with an optimal speed of convergence of order $\bigoh \parens*{\log\parens{\nRoutes} / \nRuns^{2}}$; thus it outperforms EW while maintaining the dimension-free property. 


%Therefore, Theorem~\ref{propo:AccExpoGrad} confirms that \ac{AcceEW} learns the equilibrium flows with an optimal speed of convergence of order $\bigoh \parens*{\log\parens{\nRoutes} / \nRuns^{2}}$; thus it outperforms EW while maintaining the dimension-free property.
 
% % \footnote{We can construct a routing game instance guaranteeing that any algorithm yields a convergence rate that is lower-bounded by $\Theta\parens*{1/\nRuns^{2}}$ based on similar results of \cite{nemirovski2004prox} for convex~optimization.}

% % We give the detailed proof of Theorem~\ref{propo:AccExpoGrad} in~\ref{sec:appen_acceEW} \revise{and discuss its main ideas here. First, we can prove the following lemma:
% % %
% % \begin{lemma} \label{lem:Acce_mainlem}
% %     Let \mbox{$\hreg \parens*{\flow} :=  \sum \limits_{\pair \in \pairs} \sum\limits_{\route \in \routes_\pair} \flow_{\pair, \route} \log \parens*{\flow_{\pair, \route}}$}, $\forall \flow \in \flows$, and $\flow^{\run}$ computed by Algorithm~\ref{algo:AccExpGrad} at iteration $\run$, we have
% %     \begin{equation}
% %         \cost\parens*{ \flow^\nRuns} - \cost\parens{ \flowbase} \le { 4   \smooth \bregman{\hreg}{ \flowbase}{ \flow^{\start}} } / {\parens{\nRuns - \afterstart}^2 }.\label{eq:adding} 
% %     \end{equation}
% % \end{lemma}
% % Here, $\bregman{\hreg}{\cdot}{\cdot}$ denotes the Bregman divergence \wrt $\hreg$ and \eqref{eq:adding} comes from the fact that \mbox{$\stepalt^{\nRuns-1} \bracks*{\cost \parens*{\flow^{\nRuns}} - \cost \parens*{\flowbase} } \le \bregman{\hreg}{ \flowbase}{ \flow^{\start}}$} (obtained thanks to the smoothness of $\cost$) and that when $\stepalt^{\run}$ is chosen as in Line~\ref{line:AcceEW_stepalt}-Algorithm~\ref{algo:AccExpGrad}, $\stepalt^{\nRuns-1}$ is lower bounded by the corresponding constant. Finally, since $\hreg$ is a $(1/N)$-strongly convex function on $\flows$, we obtain the convergence rate as presented in Theorem~\ref{propo:AccExpoGrad}.
% % }

% {
% Note finally that the combination of Nesterov's accelerated scheme along with the generic mirror descent template have been considered in previous works (see \eg \cite{allen2014linear,krichene2015accelerated,Xiao2010}) and the application with entropy regularizer (which induces the EW template) was also analyzed by \cite{krichene2015accelerated}. That said, as far as our knowledge goes, our work is the first application of this approach in the context of routing games with explicit convergence rates on games~parameters.
% }
% %A proof of Proposition~\ref{propo:AccExpoGrad} is given in \ref{sec:appen_acceEW}. Intuitively, the sequence $\parens*{\flow^{\run}}_{\run \in \N}$ computed by Algorithm~\ref{algo:AccExpGrad} converges toward the set of equilibrium normalized flow of the games. 
% %Moreover, the  rate of convergence of \ac{AcceEW} is in order $\bigoh \parens*{\log\parens{\nRoutes} / \nRuns^{2}}$ which is much better than that of the EW Algorithm. In an alternative perspective, it only takes at least an $\bigoh \parens*{\eps^{-1/2}}$ number of iterations of \ac{AcceEW} to obtain an $\eps$-approximate solution of \eqref{OPT1}. In fact, this order of convergence rate is optimal in term of $\nRuns$ for the class of gradient descent algorithms.\footnote{We can construct a routing game instance guaranteeing that any algorithm yields a convergence rate that is lower-bounded by $\Theta\parens*{\nRuns^{-2}}$ based on similar results of \cite{nemirovski2004prox} for convex~optimization.} Moreover, the fact that this rate of convergence is in logarithmic order in terms of $\nRoutes$---the number of paths in the network---shows the scalability of the \ac{AcceEW} Algorithm since in practice, it is often the case that $\nRoutes$ is exponentially large. 
% %We now analyze the key novelty of \ac{AcceEW}. 
% %Unlike the EW Algorithm, at each iteration, Algorithm~\ref{algo:AccExpGrad} (\ac{AcceEW} Algorithm) makes use of information of the previous iterations via the terms updated in Lines~\ref{line:AcceEW_dpoint} and~\ref{line:AcceEW_ppoint}. At each iteration $\run$, it queries the cost corresponding to $\ppointalt^{\run-1}$ (which is a convex combination of points computed in the previous iteration), observes the corresponding estimated cost and use it to proceed (see Line~\ref{line:AcceEW_dpoint}-Algorithm~\ref{algo:AccExpGrad}). 
% % Note importantly that \ac{AcceEW} is no mere direct application of existing algorithms in convex optimization to the context of routing games. The novelty of \ac{AcceEW} also lies at our choice of adaptive sequences of step-sizes $\step^{\run}$ and $\stepalt^{\run}$ (which control the exponential-weight updating step at Line~\ref{line:AcceEW_ppoint}); this allows us to have an analysis that obtains an explicit result on the convergence rate. Although \ac{AcceEW} has improved the convergence rate in the deterministic setting in comparison to the EW Algorithm, it still has the  drawback of requiring to know a priori the parameters $\ratmax$, $\length$ and $\bderiv$ to tune the parameter~$\smooth$. 


% %Finally, note that the scope of applications of \ac{AcceEW} goes beyond the context of routing games. We can generalize Algorithm~\ref{algo:AccExpGrad} to solve a general optimization problem of the form $\min_{\point \in \cvx} \obj(\point)$ ($\obj$ is a convex smooth function and \mbox{$\cvx \subset \mathbb{R}^{\dims}$} is a convex set) in which Line~\ref{line:AcceEW_ppoint} is replaced by  \mbox{$\ppoint^{\run}\! = \!\argmin \limits_{\ppoint \in \cvx} \braces*{ \stepaltalt^{\run}  \inner{\!\nabla \!\obj \parens{\ppointalt^{\run\!-\!1}}}{\ppoint \!-\! \ppoint^{\run\!-\!1} } \! +\!   \bregman{\hreg}{\ppoint}{\ppoint^{\run\!-\!1}}}$} where $\stepaltalt^{\run}:= \parens{1\!-\! \step^{\run\!-\!1}}   \stepalt^{\run\!-\!1}$ and $\bregman{\hreg}{\cdot}{\cdot}$ is the Bregman divergence \wrt a regularizer $\hreg$.\footnote{By replacing $\obj = \cost$, $\cvx = \flows$ and for any $\flow \in \flows$, \mbox{$\hreg \parens*{\flow}=  \sum_{\pair \in \pairs} \sum_{\route \in \routes_\pair}  \flow_{\pair, \route} \log \parens*{\frac{1}{\flow_{\pair, \route}}}$}, we retrieve Algorithm~\ref{algo:AccExpGrad}.} See \ref{sec:appen_acceEW} for more~details. 









 
 

==> Algorithms/AcceleWeight.tex <==
%----------------------------------------------------------------------
%%% EXPWEIGHT ALGO
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\KwIn{Smoothness parameter $\smooth = \length\bderiv$}

\textbf{Initialize}
	$\beforeinit[\dstate] \gets \zer$;\,
	$\beforeinit[\state] \gets \zer$;\,
	$\beforeinit[\step] \gets 0$;\,
	$\beforeinit[\stepalt] \gets (\nPairs \massmax \smooth)^{-1}$
	\label{line:XLEW_initial}\;

\For{$\run = \running$}
{
		set $\curr[\pstate] \gets \logit (\prev[\dstate])$
	\tcp*[r]{exploratory flow obtained from path scores}
	\label{line:XLEW_ppoint}
		set $\curr[\state] \gets \prev[\step] \prev[\state] + (1 - \prev[\step]) \curr[\pstate]$
	\tcp*[r]{average with previous state}
	\label{line:XLEW_flow}%
		set $\curr[\stepalt]
			\gets \prev[\stepalt]
			+ \beforeinit[\stepalt]/2
			+ \sqrt{\prev[\stepalt] \beforeinit[\stepalt] + (\beforeinit[\stepalt]/2)^{2}}$
	\tcp*[r]{update step-size}
	\label{line:XLEW_stepalt}
		set $\curr[\step] \gets {\prev[\stepalt]} \big/ {\curr[\stepalt]} $
	\tcp*[r]{update averaging weight} 
	\label{line:XLEW_step}
		set $\curr[\pstateavg] \gets \curr[\step] \curr[\state] + (1 - \curr[\step] ) \curr[\pstate]$
		and
		get $\curr[\signalavg] \gets \cost \parens*{\curr[\pstateavg],\curr[\sample]}$
	\tcp*[r]{route and measure costs}
	\label{line:XLEW_dpoint}
		set $\curr[\dstate]
			\gets \prev[\dstate]
			- (1 - \curr[\step]) \curr[\stepalt]\curr[\signalavg]$
	\tcp*[r]{update path scores}  
}

==> Algorithms/ExpWeight.tex <==
%----------------------------------------------------------------------
%%% EXPWEIGHT ALGO
%----------------------------------------------------------------------
% !TEX root = ../Main.tex


\textbf{Initialize} $\beforeinit[\dstate] \gets \zer$\;
\label{line:flow0}
\For{$\run = \running$}
{
	set $\curr[\state]  \gets \logit(\prev[\dstate])$
	and
	get $\curr[\signal] \gets \cost(\curr[\state],\curr[\sample])$
\tcp*[r]{route and measure costs}
\label{line:EW_flow}
	%	
	set $\curr[\dstate]  = \prev[\dstate]  - \curr[\stepalt]\curr[\signal]$
\tcp*[r]{update path scores}
\label{line:EW_dpoint} 
}

==> App-AdaPush.tex <==
For the sake of completeness, we present the distributed variants here. 


\subsection{Distributed EW Algorithm}



Here is the distributed \expweight

\begin{algorithm}[h!]
	\ttfamily
	\small
	\SetKw{Return}{Return} %Change keyword return to Return
	\SetKwInput{KwIndis}{Input at each vertex $\vertex$} %Change keyword Input
	\KwIndis{$\pairs_{\vertex}, \In{\pair}{\vertex}, , \child{\pair}{\vertex}, \parent{\pair}{\vertex}$}
	%%%%%%%%%%%%%%
	
	Initialize $\dpoint^{\beforestart}_{\vertex, \pair, \edge} = 0, \forall \pair \in \pairs_{\vertex}, \forall \edge \in \Out{\pair}{\vertex}$ at vertex $\vertex \in \vertices$ \tcp*[f]{initialize scores on outgoing edges}\; 
	%
	\For{\run =\start, \afterstart, \ldots}{
		%
		Each $\vertex \in \vertices$ resets $\push{\vertex, \pair} \gets \false$ and $\Rout{\vertex} \gets \false$ for all $\pair$\;
	
	%---------------------------	
	\While(\tcp*[f]{while there is still traffic not reaching destinations.}){$\exists \pairalt \in \pairs: \Rout{\sink{\pairalt}}= \false$}{
		%------
		%-----
		\For{\ttfamily $\vertex \in \vertices$}{
			%-----
			\For{\ttfamily $\pair \in \pairs_\vertex$ such that $\push{\vertex,\pair} = \false$}{
				$\vertex$ runs $\scorepush(\vertex, \pair, \disdstate^{\run})$ to return $\disflowpush_{\vertex, \pair}$ and update~$\push{\vertex,\pair}$,\\
				%
				then sets $\disstate^{\run}_{\vertex,\pair, \edge}   \!\gets\! \disflowpush_{\vertex, \pair, \edge}$ for $\edge \in \Out{\vertex}{\pair}$\;
			}%end while loop exists push[O_i]
			%----------
			\uIf{\ttfamily $\push{\vertex,\pair} = \true$  for all $\pair \in \pairs_\vertex$}{
				%
				%
				%
				\uIf{\ttfamily $\vertex$ receives the $\pair$-type traffic \textbf{from all} $\vparent \in \parent{\vertex}{\pair}$ and \textbf{for all} $\pair \in \pairs_\vertex$  }{
					$\vertex$ gets $\signal^{\run}_{\edge} \gets \dislate_{\edge} \parens*{\load_{\edge} \parens{\disstate^{\run}}, \sample^{\run}}$ and updates $\disdstate^{\run+1}_{\vertex, \pair, \edge} \gets \disdstate^{\run}_{\vertex, \pair, \edge} - \stepalt^{\run}  \signal^{\run}_{\edge} $ for any $\pair \in \pairs_\vertex$ and $\edge \in \Out{\vertex}{\pair}$\;
					%
					update $\Rout{\vertex} = \true$\;
				}
			} % end else 
		} %end for v \in V
	}  % end while exists Route[D_i] = 0
	} 	% end for
	\caption{Distributed \expweight} \label{algo:DisEW}
\end{algorithm}













%--------------------------------
%---------------------------------
%\subsection{Distributed \Ac{AEW} Algorithm}

% First, we need an enhanced version of score-pushing that includes the additional weights (denoted by $\sumflow{\run}$) that is involved in \ac{AEW} algorithm.
% \begin{algorithm}[ht!]
% 	\SetKw{Return}{Return} %Change keyword return to Return
% 	% 	\KwIn{A regularizer $\hreg: \R^\dims \rightarrow \cvx$}
% 	%%%%%%%%%%%%%%
% 	%
% 	\uIf(\tcp*[f]{when there is still traffic for $\vertex$ to push}){$\unpush{\vertex} \neq \emptyset$}{
% 		\For{$\pair \in \unpush{\vertex}$}{
% 			\uIf{$\vertex$ is informed of $\score_{\pair, \vertexalt}$ \textbf{from all} $\vchild \in \child{\pair}{\vertex}$}{
% 				%
% 				\lIf{$\vertex = \sink{\pair}$}{set $\score_{\pair, \vertex}:=1$ }
% 				%
% 				\lElse{compute $\score_{\pair, \vertex}:= \sum_{\vchild \in \child{\pair}{\vertex}}{ \score_{\pair, \vchild} \exp \parens*{\Dpoint_{\vertex, \pair, \edgec{\vertex}{\vchild}} } }$}
% 				%
% 				Vertex $\vertex$ informs $\score_{\pair, \vertex}$ to all $\vparent \in \parent{\pair}{\vertex}$\;
% 				%
% 				\Return{$\disflowpush_{\vertex, \pair, \edge} = \frac{1}{\sum_{\runalt=1}^{\run} \runalt} \bracks*{ \run  \exp \parens*{\Dpoint_{\vertex, \pair, \edge}} \frac{\score_{\pair, \vchild}}{\score_{\pair, \vertex}}  + \sumflow{t}_{\vertex,\pair,\edge} }$, $\forall \edge=\edgec{\vertex}{\vchild} \in \Out{\pair}{\vertex}$}\;
% 				%
% 				\textbf{Remove} $\pair$ from $\unpush{\vertex}$\;
% 			}
% 		}

% 	}
% 	%
% 	\uElse(\tcp*[f]{when $\vertex$ finished pushing all relevant traffic types}){\textbf{Update} $\push{\vertex}:= 1$ } 
% 	\caption{Score-pushing with averaging $\SPA \parens*{\vertex, \Dpoint, \sumflow, \run}$.}\label{alg:score_push}
% \end{algorithm}






%%
%%
%--------------------
%-------------------------
\subsection{Proof of \cref{thm:adapush}}

In this section, we additionally use some other notation as follows. Let $\routes^{\pair}_{\vertex : \vertexalt} \subset \routes_\pair$ denote the set of all (directed) paths in $\graph_\pair$ going from vertex $\vertex$ to vertex $\vertexalt$. 






\para{Convergence analyses} We focus on proving that for any iteration $\run$, the cost induced by the distributed flow $\disstate^{\run}$ (computed by Algorithm~\ref{alg:adapush}) is equal to the cost induced by the flow $\state^{\run}$ (computed by Algorithm~\ref{alg:AEW}). As a consequence, the potential value $\discost(\disstate^{\run})$ is equal to the potential value $\cost(\state^{\run})$ and the convergence rates obtained by \adapush are the same as that of \method. Therefore, \cref{thm:adapush} can be directly deduced from \cref{thm:AEW}.


Particularly, by induction, we first prove that $\disload_{\edge}(\disstate^{\run}) = \load_{\edge}(\state^{\run}, \forall \edge \in \edges$.












\begin{align}
	\score_{\pair, \vertex} &= \sum_{\route \in \routes^{\pair}_{\vertex:\sink{\pair}} } \prod_{\edgec{\vertexalt}{\vertexaltalt} \in \route} \exp \parens*{\disdstate^{\run}_{\vertexalt, \pair, \edgec{\vertexalt}{\vertexaltalt}}},\label{eq:lemma_chain_vertex}  \\
	%
	{\rm ~and~}       \disload_{\pair, \edge} (\disflowpush) & = \mass{\pair} \frac{\sum_{\route \in \routes_\pair \atop \route \ni \edge} \prod_{\edgec{\vertexalt}{\vertexaltalt} \in \route} \exp \parens*{\disdstate^{\run}_{\vertexalt, \pair, \edgec{\vertexalt}{\vertexaltalt}}}}      {  \sum_{\routealt \in \routes_\pair} \prod_{\edgec{\vertexalt}{\vertexaltalt} \in \routealt} \exp \parens*{\disdstate^{\run}_{\vertexalt, \pair, \edgec{\vertexalt}{\vertexaltalt}} } }. \label{eq:lemma_chain_edge} 
\end{align}



\begin{proof}
	 
	%---------
	\textit{\underline{Step 1:} Check \eqref{eq:induc_DisExpGrad} for $\run =\start$.} Fix a pair $\pair \in \pairs$ and an edge $\edgebase \in \edges_{\pair}$. From Lemma~\ref{lem:chain} and the choice of $\disdstate^{\start}_{\pair, \edge}$ (see Line~\ref{line:init_end} of Algorithm~\ref{algo:DisExpGrad}), we have
	
	\begin{equation}
		\score^{\start}_{\pair, \edgebase}    
		%
		= \frac{\sum_{\route \in \routes_\pair \atop \route \ni \edgebase} \prod_{\edge \in \route} \exp \parens*{0}}{  \sum_{\route \in \routes^{\pair}_{\source{\pair}:\sink{\pair}} } \prod_{\edge \in \route} \exp \parens*{0} }
		%
		= \frac{\sum_{\route \in \routes_\pair \atop \route \ni \edgebase}1 }{\sum_{\route \in \routes_{\pair} } 1} = \frac{\sum_{\route \in \routes_\pair \atop \route \ni \edgebase}1 }{\abs*{\routes_\pair}}. \label{eq:endingstep1-1}
	\end{equation}
	
	
	
	On the other hand, by the choice of $\flow^{\start}$ (see Line~\ref{line:flow0} of Algorithm~\ref{algo:ExpGrad}), we have
	\begin{equation}
		\sum \limits_{\route \in \routes_\pair \atop \route \ni \edge} \flow^{\start}_{\pair, \route} =  \sum \limits_{\route \in \routes_\pair \atop \route \ni \edge} \frac{\start}{\abs*{\routes_\pair}}. \label{eq:endingstep1-2}
	\end{equation}
	
	From \eqref{eq:endingstep1-1} and \eqref{eq:endingstep1-2}, we conclude that $ \sum \limits_{\route \in \routes_\pair \atop \route \ni \edgebase} \flow^{\start}_{\pair, \route} =  \score^{\start}_{\pair, \edgebase}$. This concludes Step 1. 
	
	
	
	%%%%%%
	\textit{\underline{Step 2:} Assume that \eqref{eq:induc_DisExpGrad} holds for any $\run = \afterstart, \ldots, \nRuns-1$ (with any $\pair \in \pairs$, any $\edge \in \edges_\pair$). We want to prove that it holds with $\nRuns$.} 
	
	For any $\run =\afterstart,\ldots, \nRuns-1$, any $\pair \in \pairs$ and any $\edge \in \edges_\pair$, by the induction hypothesis, we have \mbox{$\sum \limits_{\routealt \in \routes_\pair \atop \routealt \ni \edge} \flow^{\run}_{\pair, \routealt} =  \score^{\run}_{\pair, \edge}$}; therefore, for any $\route \in \routes_\pair$, from \eqref{eq:deri-cost}, we can deduce:
%	\begin{align}
%		\nabla_{\pair, \route} \cost \parens{\flow^{\run}} 
%		&=  \rat_\pair   \sum_{\edge \in \route} \bracks*{ \late_{\edge}  \parens*{ \sum_{\pairalt \in \pairs } \rat_\pairalt \sum_{\routealt \in \routes_\pairalt \atop \routealt \ni \edge} \flow^{\run}_{\pairalt, \routealt} } + \sum_{\pairalt \in \pairs } \rat_\pairalt  \sum_{\routealt \in \routes_\pairalt \atop \routealt \ni \edge} \flow^{\run}_{\pairalt, \routealt} \cdot    \derlate_{\edge}  \parens*{ \sum_{\pairaltalt \in \pairs } \rat_\pairaltalt  \sum_{\routealtalt \in \routes_\pairaltalt \atop \routealtalt \ni \edge} \flow^{\run}_{\pairaltalt, \routealtalt}}}\nonumber \\
%		%
%		&= \rat_\pair  \sum_{\edge \in \route} \bracks*{ \late_{\edge}  \parens*{ \sum_{\pairalt \in \pairs } \rat_\pairalt \score^{\run}_{\pairalt, \edge}  } + \sum_{\pairalt \in \pairs } \rat_\pairalt  \score^{\run}_{\pairalt,\edge} \cdot    \derlate_{\edge}  \parens*{ \sum_{\pairaltalt \in \pairs } \rat_\pairaltalt \score^{\run}_{\pairaltalt,\edge}}} \nonumber\\
%		%
%		&= \sum_{\edge \in \route} \grade^{\run}_{\pair, \edge} . \label{eq:derive_grade}
%	\end{align}
	Here, the last equality comes directly from \eqref{eq:define_grade}.
	
	Now, for any $\pair \in \pairs$ and $\edgebase \in \edges_\pair$, from the definition of $\flow^{\run}$ (Line~\ref{line:flow} of Algorithm~\ref{algo:ExpGrad}), we have
	%
	\begin{align}
		&\sum_{\route \in \routes_\pair \atop \route \ni \edgebase } \flow^{\nRuns}_{\pair, \route} \nonumber \\
		%
		=&\sum_{\route \in \routes_\pair \atop \route \ni \edgebase } \frac{ \flow^{\nRuns-1}_{\pair, \route}  \exp \parens*{ -\strong \nabla_{\pair, \route} \cost \parens*{\flow^{\nRuns-1}}} }{ \sum \limits_{\routealt \in \routes_\pair}   \flow^{\nRuns-1}_{\pair, \routealt} \exp \parens*{ -\strong \nabla_{\pair, \routealt} \cost \parens*{\flow^{\nRuns-1}}} }   \nonumber\\
		%
		=& \sum_{\route \in \routes_\pair \atop \route \ni \edgebase } \frac{ \frac{\flow^{\nRuns-2}_{\pair, \route} \exp \parens*{-\strong \nabla_{\pair, \route}\cost \parens*{\flow^{\nRuns-2}}}}{ \sum \limits_{\routealtalt \in \routes_\pair}   \flow^{\nRuns-2}_{\pair, \routealtalt} \exp \parens*{ -\strong \nabla_{\pair, \routealtalt} \cost \parens*{\flow^{\nRuns-2}}}  }  \exp \parens*{ -\strong \nabla_{\pair, \route} \cost \parens*{\flow^{\nRuns-1}}} }{ \sum \limits_{\routealt \in \routes_\pair}   \frac{\flow^{\nRuns-2}_{\pair, \routealt} \exp \parens*{-\strong \nabla_{\pair, \routealt}\cost \parens*{\flow^{\nRuns-2}}}}{ \sum \limits_{\routealtalt \in \routes_\pair}   \flow^{\nRuns-2}_{\pair, \routealtalt} \exp \parens*{ -\strong \nabla_{\pair, \routealtalt} \cost \parens*{\flow^{\nRuns-2}}}  } \exp \parens*{ -\strong \nabla_{\pair, \routealt} \cost \parens*{\flow^{\nRuns-1}}} }   \nonumber\\
		%
		=&    \sum_{\route \in \routes_\pair \atop \route \ni \edgebase } \frac{ \flow^{\nRuns-2}_{\pair, \route}  \exp \parens*{ -\strong \sum \limits_{\run = \nRuns-2}^{\nRuns-1}   \nabla_{\pair, \route} \cost \parens*{\flow^{\run}}}}{ \sum \limits_{\routealt \in \routes_\pair}   \flow^{\nRuns-2}_{\pair, \routealt}  \exp \parens*{ -\strong \sum \limits_{\run = \nRuns-2}^{\nRuns-1}   \nabla_{\pair, \routealt} \cost \parens*{\flow^{\run}}} }\nonumber \\     
		%
		& \qquad \qquad \vdots  \nonumber \\  
		%
		=&   \sum_{\route \in \routes_\pair \atop \route \ni \edgebase } \frac{ \flow^{1}_{\pair, \route}  \exp \parens*{ -\strong \sum \limits_{\run = 1}^{\nRuns-1}   \nabla_{\pair, \route} \cost \parens*{\flow^{\run}}}}{ \sum \limits_{\routealt \in \routes_\pair}   \flow^{1}_{\pair, \routealt}  \exp \parens*{ -\strong \sum \limits_{\run = 1}^{\nRuns-1}   \nabla_{\pair, \routealt} \cost \parens*{\flow^{\run}}} } \nonumber\\
		%
		=& \sum_{\route \in \routes_\pair \atop \route \ni \edgebase } \frac{ \frac{1}{\abs*{\routes_\pair}}  \exp \parens*{ -\strong \sum \limits_{\run = 1}^{\nRuns-1}  \sum\limits_{\edge \in \route} \grade^{\run}_{\pair, \edge} }}{ \sum \limits_{\routealt \in \routes_\pair}   \frac{1}{\abs*{\routes_\pair}} \exp \parens*{ -\strong \sum \limits_{\run = 1}^{\nRuns-1}   \sum\limits_{\edgealt \in \routealt} \grade^{\run}_{\pair, \edgealt}} }  \qquad \qquad {\rm~(from~\eqref{eq:derive_grade}~and~Line~\ref{line:flow0}~of~Algorithm~\ref{algo:ExpGrad})} \nonumber\\
		%
		=&\sum_{\route \in \routes_\pair \atop \route \ni \edgebase } \frac{ \prod\limits_{\edge \in \route} \exp \parens*{-\strong   \sum \limits_{\run = 1}^{\nRuns-1}    \grade^{\run}_{\pair, \edge} }}{ \sum \limits_{\routealt \in \routes_\pair} \sum \limits_{\edgealt \in \routealt}     \prod\limits_{\run = 1}^{\nRuns-1}     \exp\parens*{ -\strong \grade^{\run}_{\pair, \edgealt}} }. \label{eq:ending_proof_induc_1}
	\end{align}
	Finally, from Line~\ref{line:grade} of Algorithm~\ref{algo:DisExpGrad}, for any $\pair \in \pairs$ and any $\edge \in \edges_\pair$, we have\footnote{Note that $\disdstate^{\start}_{\pair, \edge} = 0, \forall \pair \in \pairs, \forall \edge \in \edges_\pair$.} 
	\begin{equation*}
		\disdstate^{\nRuns}_{\pair, \edge} =\disdstate^{\nRuns-1}_{\pair, \edge} - \strong \grade^{\nRuns-1}_{\pair, \edge} = \disdstate^{\nRuns-2}_{\pair, \edge} -\strong \parens*{ \grade^{\nRuns-2}_{\pair, \edge} + \grade^{\nRuns-1}_{\pair, \edge}} = \ldots = \disdstate^{\start}_{\pair, \edgebase} - \strong \sum_{\run=\start}^{\nRuns-1} \grade^{\run}_{\pair, \edge} = - \strong \sum_{\run=\start}^{\nRuns-1} \grade^{\run}_{\pair, \edge}.
	\end{equation*}
	Combining this with Lemma~\ref{lem:chain}, for any $\pair \in \pairs$ and $\edgebase \in \edges_\pair$, we have:
	\begin{align}
		\score^{\nRuns}_{\pair,\edgebase} = \frac{\sum_{\route \in \routes_\pair \atop \route \ni \edgebase} \prod_{\edge \in \route} \exp \parens*{\disdstate^{\nRuns}_{\pair, \edge} }}{ \sum_{\routealt \in \routes_\pair} \prod_{\edgealt \in \routealt} \exp \parens*{\disdstate^{\nRuns}_{\pair, \edgealt}}} =   \frac{\sum_{\route \in \routes_\pair \atop \route \ni \edgebase} \prod_{\edge \in \route} \exp \parens*{- \strong \sum_{\run=1}^{\nRuns-1} \grade^{\run}_{\pair, \edge}  }}{ \sum_{\routealt \in \routes_\pair} \prod_{\edgealt \in \routealt} \exp \parens*{- \strong \sum_{\run=1}^{\nRuns-1} \grade^{\run}_{\pair, \edgealt}}} . \nonumber
	\end{align}
	Combining this with \eqref{eq:ending_proof_induc_1}, we concludes that $\score^{\nRuns}_{\pair, \edgebase} = \sum_{\route \in \routes_\pair \atop \route \ni \edgebase} \flow^{\nRuns}_{\pair, \route}$ for any $\pair \in \pairs$ and $\edgebase \in \edges_\pair$. We finish the proof of \eqref{eq:induc_DisExpGrad}.
	
	
%	Therefore, at any iteration $\run \ge 1$, the output $\nflowe^{\run}$ of Algorithm~\ref{algo:DisExpGrad} corresponds to the output $\flow^{\run} \in \flows$ of Algorithm~\ref{algo:ExpGrad}; thus, $\nflowe^{\run} \in \nflowes$. Moreover, apply Proposition~\ref{propo:DisExpoGrad}, under Assumptions~\ref{assum:cvx-con}, \ref{assum:deriv} and \ref{assum:bound}, for any $\nflowebase \in \nflowes$ (corresponding to $\flowbase \in \flows$), we~have:
%	\begin{align*}
%		\coste \parens*{\frac{1}{\nRuns} \sum_{\run =1}^{\nRuns} \nflowe^\run } - \coste \parens{\nflowebase} \le   \frac{1}{\nRuns} \sum_{\run =1}^{\nRuns} \bracks*{ \coste \parens{\nflowe^\run} - \coste \parens{\nflowebase}} =  \frac{1}{\nRuns} \sum_{\run =1}^{\nRuns} \bracks*{ \cost \parens{\flow^\run} - \cost \parens{\flowbase}} \le  \eps , 
%	\end{align*}
%	where \mbox{$\nRuns := \ceil*{\frac{ 2 \lips^2  \nPairs \log\parens*{\nRoutes/ \nPairs}}{\eps^2}} $}, $\strong =  \sqrt{\frac{2 \nPairs \log \parens*{\frac{\nRoutes}{\nPairs} }}{ \lips^2 \nRuns}}$ and $\lips := \ratmax \length  \cdot \parens*{\ub +  \nPairs \bderiv  \ratmax }$.
%	
	
	
	
\end{proof}



==> App-Aux.tex <==
%----------------------------------------------------------------------
%%% APP: GAMEFORM
%----------------------------------------------------------------------
% !TEX root = ./Main.tex

 
 \begin{centering}
 	\begin{table}[htb!]
 		\caption{Table of Notation}
 		\captionsetup{justification=centering}
 		%
 		\begin{tabular}{r c p{12cm} }
 			%\toprule
 			\multicolumn{3}{c}{\underline{Notation related to network structures}}\\
			$\graphall$ & $\defeq$ &  graph with vertices set $\vertices$ and edges set $\edges$
			\\
			$\pairs$  & $\defeq$ & set of all \ac{OD} pairs
			\\ 
 			$\routes^\pair$ & $\defeq$ & set of all paths going from $\source{\pair}$ to $\sink{\pair}$  
 			\\
 			$\graph^{\pair}(\vertices_\pair, \edges_\pair)$ & $\defeq$ &  sub-graph corresponding to \ac{OD} pair $\pair$
 			\\
 			$\In{\vertex}{\pair}$ and $\Out{\vertex}{\pair}$ & $\defeq$ & the set of incoming edges and the set of outgoing edges of $\vertex$ in $\graph_\pair$
 			\\
 			$\child{\vertex}{\pair}$ and $\parent{\vertex}{\pair}$ & $\defeq$ & the set of direct successors and the set of direct predecessors  of $\vertex$ in $\graph_\pair$
 			\\
 			%
			\multicolumn{3}{c}{\underline{Notation related to routing games}}\\
 			$\flow$, $\flows$ & $\defeq$ & flow profile and the set thereof\\
 			$\load_{\edge}$  & $\defeq$ & the load of traffic on edge $\edge$\\				
 			\bottomrule
 		\end{tabular}
 		\label{table:notation}
 	\end{table}
 \end{centering}












%
%
%\subsection{Gradient of $\cost$} 
%\label{sec:app-grad_cost}
%We notice that under \cref{asm:late}, $\late_\edge, \edge \in \edges$ are continuous and non-decreasing functions. As a trivial consequence, $\cost$ is a convex function. Moreover, it is differentiable and when $\sample$ is generated randomly, for any $\pair \in \pairs$ and any path $\route \in \routes^\pair$, by recalling that \mbox{$\load_{\edge}(\flow) = \sum_{\pair \in \pairs} \sum_{\route \in \routes^\pair \atop \route \ni \edge } \flow_{\pair, \route}$} and applying the dominated convergence theorem, we have:
%
%\begin{align}
%	\dis \frac{\partial \cost}{\partial \flow_{\pair, \route}} \parens*{\flow} \!=\! \ex \bracks*{\frac{\partial \pot_{\sample}}{\partial \flow_{\pair, \route}} \parens{\flow}  } \!=\!  \ex \bracks*{ \frac{ \sum \limits_{\edge \in \edges} \int_{0}^{\load_\edge(\flow)} \late_{\edge} \parens{\real, \sample} \dd \real}{\partial \flow_{\pair, \route}}   } = &  \ex \bracks*{ \sum_{\edge \in \edges} \frac{\partial\load_{\edge}(\flow)}{\partial \flow_{\pair, \route}} \late_{\edge} \parens*{\load_{\edge}(\flow), \sample}} \nonumber\\
%	%
%	=  & \ex \bracks*{\sum_{\edge \in \route}  \late_{\edge} \parens*{\load_{\edge}(\flow), \sample} } \nonumber\\
%	%
%	= & \barlate_{\route} (\flow). \label{eq:grad_cost}
%\end{align}
%%
%Using the notation $\late(\flow, \sample)$ to present the (random) vector of costs at flow $\flow$ and $\sample$, we can also rewrite that $\grad \cost(\flow) = \ex \bracks*{\late (\flow, \sample) }$ for any $\flow \in \flows$. 

%
%
%
%--------------------------------------------
%\subsection{Auxiliary notions}
%\label{app:preli-notion}
%
%Throughout the remainder of this work, we use the notation $\inner{\cdot}{\cdot}$ to denote the Euclidean inner product of two vectors. We also denote $\prob\parens*{E}$ the probability of an event $E$. We say that $\hreg$ is \emph{$\strong$-strongly} convex over $\cvx$ \wrt $\norm{\cdot}$ if and only if for \mbox{$\point, \pointalt \in \cvx$}, we have \mbox{$\hreg\parens{\point} - \hreg\parens{\pointalt} - \inner{\subgrad}{ \point - \pointalt} \ge \frac{\strong}{2} \norm{\point - \pointalt}^2$} for any $\subgrad \in \partial \hreg \parens{\pointalt}$ (\ie $\subgrad$ is a sub-gradient of $\hreg$ at~$\pointalt$).
%
%
%%\paragraph{Entropy regularizer.} In the remainders of this paper, we recurrently work with the function 
%%It has several properties of interests as~follows:
%%\begin{itemize}[leftmargin = *]
%%	\item For any $\flow \in \flows$, $\hreg(\flow) \le \sum_{\pair \in \pairs} \sum_{\route \in \routes} \flow_{\pair, \route} \log (\mass{\pair}) \le \masssum \log(\massmax)$.
%%	%
%%	\item  $\hreg$ is a $\frac{1}{\strong}$-strongly convex function on $\flows$ \wrt the $\norm{\cdot}_1$ norm where we denote $\strong:= \massmax \nPairs$.\footnote{Consider the functions $\hreg_{\pair}((\flow_{\pair, \route})_{\route \in \routes^\pair}) = \sum_{\route \in \routes^\pair} \flow_{\pair, \route} \log (\flow_{\pair, \route})$, it is trivial to see that $\hreg_\pair (\cdot)$ is $\frac{1}{\mass{\pair}}$-strongly convex on $\flows_\pair = \braces*{ (\flow_{\pair, \route})_{\route \in \routes^\pair}: \sum_{\route \in \routes^\pair} \flow_{\pair, \route} = \mass{\pair}}$ \wrt to the norm $\norm{\cdot}_1$. Therefore, for any $\flow, \flowalt \in \flows$ and a sub-gradient $\subgrad \in \partial \hreg(\flowalt)$, we have $\hreg(\flow) = \sum_{\pair \in \pairs}  \hreg_{\pair} (  (\flow_{\pair, \route})_{\route \in \routes^\pair} ) \ge \hreg(\flowalt) + \inner{\subgrad}{\flow - \flowalt} + \sum_{\pair \in \pairs} \frac{1}{2\mass{\pair}} \parens*{ \sum_{\route \in \routes} \abs*{ \flow_{\pair, \route} - \flowalt_{\pair, \route} } }^2 \ge \hreg(\flowalt) + \inner{\subgrad}{\flow - \flowalt} + \frac{1}{2 \massmax \nPairs} \norm{\flow - \flowalt}_1^2$ due to Cauchy-Schwarz~inequality.}
%%	%
%%	\item The Fenchel conjugate of $\hreg$---denoted by $\hreg^{\ast}$---and its gradient at an arbitrary $\dpoint \in \R^{\nRoutes}$ are:
%%	%
%%	\begin{align*}
%%		\hreg^{\ast}(\dpoint) & :=  \max_{\flow \in \flows} \inner*{\flow}{\dpoint} - \hreg(\flow) =\sum_{\pair \in \pairs} \mass{\pair} \log \parens*{\sum \limits_{\routealt \in \routes^\pair} \exp \parens*{ \dpoint_{\pair,\routealt}}}, \\
%%		%
%%		\nabla \hreg^{\ast} (\dpoint) & = \parens*{ \mass{\pair} \frac{\exp(\dpoint_{\pair, \route})}{ \sum \limits_{\routealt \in \routes^\pair} \exp(\dpoint_{\pair, \routealt}) }}_{\pair \in \pairs \atop \route \in \routes^\pair}.
%%	\end{align*}
%%\end{itemize} 
%
%
%
%%
%% 
%%
%%\paragraph{KL divergence.} Induced from the entropy regularizer $\hreg$, we also define the Kullback–Leibler (KL) divergence between any flows $\flow, \flowalt \in \flows$ as follows: 
%%\begin{equation*}
%%	\dkl{\flow}{\flowalt } := \dis \sum_{\pair \in \pairs} \sum_{\route \in \routes^{\pair}} \flow_{\pair, \route} \log \parens*{ \frac{\flow_{\pair, \route}}{\flowalt_{\pair, \route}}}.
%%\end{equation*}
%%In other words, $	\dkl{ \flow}{\flowalt } = \hreg(\flow) - \hreg(\flowalt) - \inner*{\grad \hreg (\flowalt)}{\flow - \flowalt}$. In the remainders of this work, we will also regularly use the following trivial equality regarding the KL-divergence:
%%%
%%\begin{equation}
%%	\dkl{\flow}{\flowaltalt} = \dkl{\flow}{\flowalt} + \dkl{\flowalt}{ \flowaltalt} + \sum_{\pair \in \pairs} \sum_{\route \in \routes^\pair} \parens*{\flowalt_{\pair, \route} - \flow_{\pair, \route}} \log \parens*{\frac{\flowaltalt_{\pair,\route}}{\flowalt_{\pair, \route}}}  . \label{eq:BregmanTriangle}
%%\end{equation}
%%%
%%
%%%\paragraph{Bregman divergence.} Given a differentiable function $g: \cvx \rightarrow \R$, the Bregman-divergence associated with $g$ for $\point, \pointalt \in \cvx$ is \mbox{$\bregman{g}{\point}{\pointalt} = g\parens{\point} - g\parens{\pointalt} - \inner{\nabla g \parens{\pointalt}}{ \point - \pointalt}$}.
%%
%%
%%
%%\paragraph{Fenchel Coupling.} The \emph{Fenchel coupling} between $\flow \in \flows$ and $\dpoint \in \R^{\nRoutes}$ \wrt the regularizer $\hreg$ is defined as follows: 
%%\begin{equation}
%%	\fench \parens*{\flow, \dpoint} = \hreg \parens*{\flow} + {\hreg^*} \parens*{\dpoint} - \inner*{\flow}{\dpoint}. \label{eq:fench_coupl}
%%\end{equation}
%% 
%%
%% 
%%
%%
%
%
%
%
%
%
%
%
%
%
%
%\paragraph{Smoothness alternative definition.} In previous sections, we use the definition that \mbox{$\obj: \cvx \rightarrow \mathbb{R}$} is a $\smooth$-smooth convex function over $\cvx \subset \mathbb{R}^{\dims}$ \wrt the $\norm{\cdot}$ norm if and only if \mbox{$\dnorm{\nabla \obj \parens*{ \point} - \nabla \obj \parens*{\pointalt}} \le {\smooth} \norm{ \point - \pointalt}, \forall \point, \pointalt \in {\cvx}$}. This is also equivalent to the following conditions:
%\begin{equation}
%	0 \le \obj \parens*{\point} - \obj \parens*{\pointalt} - \inner{\nabla \obj \parens{\pointalt}}{\point - \pointalt}  \le  \frac{\smooth}{2} \norm{\point - \pointalt}^2, \forall \point, \pointalt \in \cvx.
%\label{eq:smooth-alter}
%\end{equation}
%%
%
%
%\begin{proof}
%While the first inequality in~\eqref{eq:smooth-alter} is trivial from the convexity of $\obj$, the second inequality can be proved by applying the mean value theorem as follows:
%\begin{align*}
%	& \obj \parens*{\point} - \obj \parens*{\pointalt} - \inner{\nabla \obj \parens{\pointalt}}{\point - \pointalt}    \\
%   = & \int \limits_{0}^1 \inner{\nabla \obj \parens*{\pointalt + \real (\point - \pointalt)}  }{\point - \pointalt} \dd \real - \int \limits_{0}^1 \inner{\nabla \obj \parens{\pointalt}  }{\point - \pointalt}\dd \real  \\
%	%
%	 \le &\int \limits_{0}^1 \dnorm{ \nabla \obj \parens*{\pointalt + \real (\point - \pointalt)} - \nabla \obj \parens{\pointalt}  } \cdot \norm{ \point - \pointalt} \dd \real \tag*{(by Cauchy-Schwarz inequality)}\\
%	%
%	\le & \norm{ \point - \pointalt} \int \limits_{0}^1 \smooth \norm{ \parens*{\pointalt + \real (\point - \pointalt)} - \pointalt  }  \dd \real\\
%	%
%	 = & \frac{ \smooth }{2}\norm{ \point - \pointalt}^2.
%\end{align*}
%\end{proof}
%



       









==> App-Disflow.tex <==
In this section, we present the proof of \cref{prop:mulflow}. For the sake of brevity, we introduce the notation $\head{\edge}$ to denote the head vertex of an edge $\edge$.  
 
 \para{Proof of Result~\textit{(i)} in \cref{prop:mulflow}}
 
	 {To prove that $\mflow{\disflow}$ is a feasible flow}, we justify the condition $\sum_{\route \in \routes_\pair} \mflow{\disflow}_{\pair, \route} =\mass{\pair}$ for any $\pair$. To do this, we label the vertices in $\graph^\pair$ by $\vertex^{i}_1, \vertex^{i}_2, \ldots, \vertex^{i}_{\abs{\vertices^\pair}}$ in a reversed topological ordering, \ie  $\vertex^{\pair}_1 = \sink{\pair}$, $\vertex^{\pair}_{\abs{\vertices^\pair}} = \source{\pair}$ and if there exists an edge in $\graph^\pair$ going from $\vertex^{\pair}_k$ to $\vertex^{\pair}_{k^{\prime}}$, then $k > k^{\prime}$. Note that such (reversed) topological ordering is available since $\graph^\pair$ is a DAG according to \cref{asm:DAG}. Let $\routes^{\pair}_{\vertex, \vertexalt}$ denotes the set of paths in $\graph^\pair$ going from vertex $\vertex \in \vertices^\pair$ to vertex $\vertexalt \in \vertices^\pair$. Let us define $H^\pair \bracks{\vertex} \defeq  	\sum_{\route \in \routes^{\pair}_{\vertex, \sink{\pair}}}  \prod_{\edge \in \route } \disflow_{\head{\edge}, \pair, \edge} $.

	We aim to prove that for any $k=2,\ldots, \abs{\vertices^\pair}$, we have
	\begin{equation}\label{eq:mulflow_1}
 	 H^{\pair} \bracks{\vertex^{\pair}_{k}} = 1.
	\end{equation}
	%
	We do this by induction. First, due to our labeling process, $\child{\vertex^{\pair}_{2}}{\pair} = \braces*{ {\sink{\pair}}}$, \ie $\sink{\pair}$ is the \emph{only} direct successor in $\graph^\pair$ of $\vertex^{\pair}_{2}$, thus, the set of its outgoing edges is $\Out{\vertex^{\pair}_{2}}{\pair} = \braces*{ \edgec{\vertex^{\pair}_{2}}{\sink{\pair}}} $. Therefore, by definition of the outgoing flow, we have $\disflow_{\vertex^{\pair}_{2}, \pair, \edgec{\vertex^{\pair}_{2}}{\sink{\pair}}}   = \sum_{\edge \in \Out{\vertex^{\pair}_{2}}{\pair} } \disflow_{\vertex^{\pair}_{2}, \pair, \edge} = 1$ and as a consequence, $H^{\pair} \bracks{\vertex^{\pair}_2}= \disflow_{\vertex^{\pair}_{2}, \pair, \edgec{\vertex^{\pair}_{2}}{\sink{\pair}}} =1$. Now, assume that \eqref{eq:mulflow_1} holds for $k=1,\ldots, K-1$ which implies that $H^{\pair} \bracks*{\vertexalt} = 1, \forall \vertexalt \in \child{\pair}{\vertex^{\pair}_{K}}$, we have:
	\begin{equation*}
		H^\pair \bracks*{\vertex^{\pair}_{K}}	= \sum_{\vertexalt \in \child{\pair}{\vertex^{\pair}_K} } \disflow_{\vertex^{\pair}_K, \pair, \edgec{\vertex^{\pair}_K}{\vertexalt}} \cdot H^{\pair} \bracks*{\vertexalt} = \sum_{\vertexalt \in \child{\pair}{\vertex^{\pair}_K} } \disflow_{\vertex^{\pair}_K, \pair, \edgec{\vertex^{\pair}_K}{\vertexalt}} =1 \qquad \textrm{(by definition of outgoing flows)}.
	\end{equation*}
	Therefore, \eqref{eq:mulflow_1} holds with $k = K$ and we conclude that it holds with any $k=1,\ldots, \abs{\vertices^\pair}$. Recall that $\vertex^{\pair}_{\abs{\vertices^\pair}} = \source{\pair}$, we have $H^{\pair} \bracks{\source{\pair}}=1$. 
	
	
	Therefore, by definition of the multiplicative flow $\mflow{\disflow}$, we have $\sum_{\route \in \routes_\pair} \mflow{\disflow}_{\pair, \route} =  \mass{\pair} \sum_{\route \in \routes_\pair} \prod_{\edge  \in \route} \disflow_{\head{\edge}, \pair, \edge }  = \mass{\pair} H^{\pair} \bracks{\source{\pair}} = \mass{\pair}$. This concludes that $\mflow{\disflow}$ is a feasible flow.  \qed


%
%
%
%----------
\para{Proof of Result~\textit{(ii)} in \cref{prop:mulflow}}	
	
	Now, {we prove that the edge loads induced by $\disflow$ and $\mflow{\disflow}$ are the same}. First, recall that, by definition, the mass of $\pair$-type traffic arriving at a vertex $\vertex$ is $\dis \ar_{\vertex, \pair}(\disflow) = \sum_{\edgealt \in \In{\vertex}{\pair}} \disload_{\pair, \edgealt}(\disflow) = \mass{\pair} \sum_{\route \in \routes^{\pair}_{\source{\pair}, \vertex} } \prod_{\edgealtalt \in \route}\disflow_{\head{\edgealtalt}, \pair, \edgealtalt } $. Therefore, for any vertex $\vertex \in \vertices^\pair$ and a successor $\vchild \in \child{\vertex}{\pair}$, the edge $\edge = \edgec{\vertex}{\vchild}$ satisfies:
	%
	\begin{align*}
	\disload_{\pair, \edge}(\disflow) = \ar_{\vertex, \pair}(\disflow) \cdot \disflow_{\vertex, \pair, \edge} 	& =  \ar_{\vertex, \pair}(\disflow) \cdot \disflow_{\vertex, \pair, \edge}  \cdot H^{\pair} \bracks{\vchild} \tag*{(due to \eqref{eq:mulflow_1})}\\
	%
	& = \mass{\pair} \parens*{\sum_{\route \in \routes^{\pair}_{\source{\pair}, \vertex} }  \prod_{\edgealtalt  \in \route}\disflow_{\head{\edgealtalt}, \pair, \edgealtalt }}  \cdot \disflow_{\vertex, \pair, \edgec{\vertex}{\vertexalt}} \cdot \parens*{\sum_{\routealt \in \routes^{\pair}_{\vchild, \sink{\pair}} }  \prod_{\edgealt  \in \routealt}\disflow_{\head{\edgealt}, \pair, \edgealt }} \\
	%
	&  =  \mass{\pair} \sum_{\route \in \routes_\pair \atop \route \ni \edge} \prod_{\edgealt \in \route}\disflow_{\head{\edgealt}, \pair, \edgealt } \\
	%
	& = \sum_{\route \in \routes_\pair \atop \route \ni \edgec{\vertex}{\vertexalt}} \mflow{\disflow}_{\pair, \route}\\
	%
	& =\load_{\pair, \edge}(\mflow{\disflow}). 
	\end{align*}

\qed
	 
	
 











==> App-GameForm.tex <==
%----------------------------------------------------------------------
%%% APP: GAMEFORM
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


%\subsection{Proof of \cref{propo:BMW}}

%
% we~compute:
%\begin{align}
%%    \nabla_{\pair, \route} \cost \parens*{\flow} :=
%    \dis \frac{\partial \cost}{\partial \flow_{\pair, \route}} \parens*{\flow} \!=\! \ex_{\sample} \bracks*{\frac{\partial \Phi}{\partial \flow_{\pair, \route}} \parens{\flow, \sample}  } & = \ex_{\sample}  \bracks*{  \sum_{\edge \in \edges} \frac{\partial \parens*{\sum \limits_{\edge \in \edges} \int_{0}^{\load_\edge(\flow)} \late_{\edge} \parens{\real, \sample} \dd \real}}{ \partial \flow_{\pair, \route}}(\flow, \sample) }  \nonumber \\ 
%    %
%    & = \ex_{\sample}  \bracks*{  \sum_{\edge \in \edges}  {\late_{\edge} \parens*{\load_{\edge}(\flow), \sample}} \frac{\partial \parens*{\sum \limits_{\pairalt \in \pairs} \sum \limits_{\routealt \in \routes^\pairalt \atop \routealt \ni \edge} \flow_{\pairalt, \routealt} }}{\partial\flow_{\pair, \route}}  } \nonumber\\
%    %
%    & = \ex_{\sample} \bracks*{\sum_{\edge \in \route}  \late_{\edge} \parens*{\load_{\edge}(\flow), \sample}  }\nonumber\\ 
%    %
%    & = \barlate_{\route} (\flow). \label{eq:grad_rosenthal}
%\end{align}
%














==> App-NumExp.tex <==


The code of our numerical experiments are available at \url{https://github.com/Anonymous-GT11/NumExperiments_AdaptiveRouting}.


For illustrating the convergence properties of the \expweight, \ac{XLEW} and \ac{AEW}~algorithms, we present below more experimental results, in addition to the ones discussed in \cref{sec:numerics}. Particularly, in \cref{sec:appen_stochastic}, we report the experiments conducted in a stochastic~setting and in \cref{sec:appen_static}, we report the experiments done in a static environment.







%
%
%---------------------------
\subsection{Performance in the stochastic regime}
\label{sec:appen_stochastic}

In this section, we work with the stochastic regime as described in \cref{sec:numerics}, \ie in a game with stochastically perturbed observations. \cref{thm:AEW} guarantees that \ac{AEW} converges at an $\bigoh(1/ \sqrt{\nRuns})$ rate. Since \cref{thm:AEW} is our core result, we re-justify it by plotting out the evolution of the term $\sqrt{\nRuns} \cdot \Delta_{\textrm{\ac{AEW}}}(\nRuns)$ (defined in \cref{sec:numerics}). We also plot out $\sqrt{\nRuns} \cdot \Delta_{\expweight}(\nRuns)$, $\sqrt{\nRuns} \cdot \Delta_{\textrm{\ac{XLEW}}}(\nRuns)$ for the sake of comparison and report all of these results in Figure~\ref{fig:t_sqrt}.



Figure~\ref{fig:t_sqrt} shows that $\sqrt{\nRuns} \cdot \Delta_{\textrm{\ac{AEW}}}(\nRuns)$ approaches a horizontal line as $\nRuns$ increases. This re-confirms that the convergence rate of \ac{AEW} is $\bigoh(1/ \sqrt{\nRuns})$. On the other hand, the divergence of $\sqrt{\nRuns} \cdot \Delta_{\textrm{\ac{XLEW}}}(\nRuns)$ confirms once again that \ac{XLEW} does not converge in this setting. 



\begin{figure}[ht!]
	\centering
	\begin{tikzpicture}
		\node (img){\includegraphics[height = 0.18\textheight]{Figures/stochastic_t2.png}};
		\node[below=of img, node distance=0cm, yshift=1.2cm, xshift =0.2cm] {\scriptsize${\nRuns}$};
		\node[left=of img, node distance=0cm, rotate=90, anchor=center,xshift=0cm, yshift=-1.0cm] {\scriptsize$\sqrt{\nRuns} \cdot \Delta(\nRuns)$};
	\end{tikzpicture}
	\caption{\centering The order of the convergence rates in a stochastic environment.}    \label{fig:t_sqrt}
\end{figure}




In the experiment reported in Figure~\ref{fig:stoch} and Figure~\ref{fig:t_sqrt}, the induced costs on each edge $\edge$ at each time epoch $\run$ is perturbed by a noise $\sample^{\nRuns}_{\edge}$ that is drawn independently from the normal distribution $\mathcal{N}(0,10)$. Now, to study the effect of noises on the performance of the algorithms, we also re-run this experiment in a ``noisier" setting: the noise $\sample^{\nRuns}_{\edge}$ is generated from $\mathcal{N}(0,50)$ for any $\nRuns$ and any $\edge$. We report the results in Figure~\ref{fig:noise}. At a high-level, we see that \ac{AEW} is more stable in the presence of noise with high-variance than \expweight (or \ac{XLEW}).




\begin{figure}[t]
	\centering
	\begin{subfigure}[b]{.48\linewidth}
		\begin{tikzpicture}
			\node (img){\includegraphics[height = 0.18\textheight]{Figures/noise.png}};
			\node[below=of img, node distance=0cm, yshift=1.25cm, xshift =0.2cm] {\scriptsize${\nRuns}$};
			%	 		\node[below=of img, node distance=0cm, yshift=1cm, xshift =0.2cm] {\textit{(a)} In the \textbf{stochastic} regime};
			\node[left=of img, node distance=0cm, rotate=90, anchor=center,xshift=0cm, yshift=-1.1cm] {\scriptsize${\Delta(\nRuns)}$};
		\end{tikzpicture}
		%\includegraphics[width=\textwidth]{Figures/stochastic.png}
		\caption{Evolution of $\Delta(\nRuns)$}
	\end{subfigure}%
	%
	\begin{subfigure}[b]{.48\linewidth}
		\begin{tikzpicture}
			\node (img){\includegraphics[height = 0.18\textheight]{Figures/noise_t2.png}};
			\node[below=of img, node distance=0cm, yshift=1.2cm, xshift =0.2cm] {\scriptsize${\nRuns}$};
			%	 		\node[below=of img, node distance=0cm, yshift=0.9cm, xshift =0.2cm] {\textit{(b)} In the \textbf{static} regime};
			\node[left=of img, node distance=0cm, rotate=90, anchor=center,xshift=0cm, yshift=-1.1cm] {\scriptsize${\sqrt{\nRuns} \cdot \Delta(\nRuns)}$};
		\end{tikzpicture}
		%\includegraphics[width=\textwidth]{Figures/stationary.png}%
		\caption{Evolution of $\sqrt{\nRuns} \cdot \Delta(\nRuns)$}

	\end{subfigure}
	\vspace{-.5ex}
	\caption{\centering The convergence speed of \expweight, \ac{XLEW} and \ac{AEW} in the stochastic regime \emph{with high-level of noises}.}
	\vspace{1ex}
	\label{fig:noise}
\end{figure}


\begin{figure}[htb!]
	\centering
	\begin{tikzpicture}
		\node (img){\includegraphics[height = 0.18\textheight]{Figures/stationary_t2.png}};
		\node[below=of img, node distance=0cm, yshift=1.3cm, xshift =0.2cm] {\scriptsize${\nRuns}$};
		\node[left=of img, node distance=0cm, rotate=90, anchor=center,xshift=0cm, yshift=-1.0cm] {\scriptsize$\nRuns^2 \cdot {\Delta(\nRuns)}$};
	\end{tikzpicture}
	\caption{\centering The order of the convergence rates in the static regime.}    \label{fig:t_square}
\end{figure}

\begin{figure}[h!]
	\centering
	\begin{subfigure}[b]{.48\linewidth}
		\begin{tikzpicture}
			\node (img){\includegraphics[height = 0.18\textheight]{Figures/EMA_stationary.png}};
			\node[below=of img, node distance=0cm, yshift=1.25cm, xshift =0.2cm] {\scriptsize${\nRuns}$};
			%	 		\node[below=of img, node distance=0cm, yshift=1cm, xshift =0.2cm] {\textit{(a)} In the \textbf{stochastic} regime};
			\node[left=of img, node distance=0cm, rotate=90, anchor=center,xshift=0cm, yshift=-1.0cm] {\scriptsize${\Delta(\nRuns)}$};
		\end{tikzpicture}
		%\includegraphics[width=\textwidth]{Figures/stochastic.png}
		\caption{Eastern-Massachusetts network: 74 vertices, 258 edges; we choose $\nPairs = 50$ O/D pairs, each of which is assigned with $10$ shortest paths; the total paths in used is $\nRoutes = 500$.}
	\end{subfigure}%
	%
	\quad 
	\begin{subfigure}[b]{.48\linewidth}
		\begin{tikzpicture}
			\node (img){\includegraphics[height = 0.18\textheight]{Figures/Austin_stationary.png}};
			\node[below=of img, node distance=0cm, yshift=1.2cm, xshift =0.2cm] {\scriptsize${\nRuns}$};
			%	 		\node[below=of img, node distance=0cm, yshift=0.9cm, xshift =0.2cm] {\textit{(b)} In the \textbf{static} regime};
			\node[left=of img, node distance=0cm, rotate=90, anchor=center,xshift=0cm, yshift=-1.1cm] {\scriptsize${ \Delta(\nRuns)}$};
		\end{tikzpicture}
		%\includegraphics[width=\textwidth]{Figures/stationary.png}%
		\caption{Austin network: 7388 vertices, 18961 edges; we choose $\nPairs =5$ O/D pairs which is assigned with $10$ shortest paths; the total paths in used is $\nRoutes = 50$.}
		
	\end{subfigure}
	\vspace{-.5ex}
	\caption{\centering The convergence speed of \expweight, \ac{XLEW} and \ac{AEW} algorithms in the static regime in Eastern-Massachusetts and Austin networks.}
	\vspace{1ex}
	\label{fig:extra_network}
\end{figure}




%
%
%
%---------------------------
\subsection{Performance in the static regime}
\label{sec:appen_static}
%
In this section, we work with the static setting. SiouxFalls is a famous network that is often used as a benchmark in the field and we reported, in \cref{sec:numerics}, the performance of the \expweight, \ac{XLEW} and \ac{AEW} algorithms on this network with data extracted from the real data set \cite{dataset2021}. To support further this numerical experiments and to re-justify the theoretical convergence rates guaranteed in \cref{thm:expweights} and \cref{thm:AEW}, we plot out $\nRuns^2 \cdot \Delta_{\expweight}(\nRuns)$, $\nRuns^2 \cdot \Delta_{\textrm{\ac{XLEW}}}(\nRuns)$ and $\nRuns^2 \cdot \Delta_{\textrm{\ac{AEW}}}(\nRuns)$. These results are reported in Figure~\ref{fig:t_square}. It shows that $\nRuns^2 \cdot \Delta_{\textrm{\ac{XLEW}}}(\nRuns)$ and $\nRuns^2 \cdot \Delta_{\textrm{\ac{AEW}}}(\nRuns)$ approach horizontal lines as $\nRuns$ increases; this confirms that \ac{XLEW} and \ac{AEW} converge at an $\bigoh(1/ \nRuns^2)$ rate which are in consistent with \cref{thm:acceleweight} and~\cref{thm:AEW}. On the other hand, $\nRuns^2 \cdot \Delta_{\expweight}(\nRuns)$ increases (almost) linearly; this demonstrates that the \expweight algorithm fails to achieve an $\bigoh(1/\nRuns^2)$-convergence rate in this setting. The slow-convergence of \ac{XLEW} with bad-tuned step-sizes (\eg when $\stepalt^{0}=1\mathrm{e}{-07}$) is also re-confirmed in Figure~\ref{fig:t_square}

















Finally, we show in Figure~\ref{fig:extra_network} the experiments results with respected to several other networks in the Transportation Networks data set (provided by \citep{dataset2021}) that are larger than SiouxFalls. We observe that, at a high level, the performance of \expweight, \ac{XLEW} and \ac{AEW} in these networks is similar to that in the SiouxFalls network. 











==> App-acceleweights.tex <==
%----------------------------------------------------------------------
%%% APP: GAMEFORM
%----------------------------------------------------------------------
% !TEX root = ./Main.tex

In this section, we provide the proof of Proposition~\ref{propo:potential} showing the smooth-continuity of the function $\cost$, then we provide the proof of Theorem~\ref{theo:acceleweight} showing the convergence properties of the \acl{AcceEW} algorithm.

%
%
%
%------------------------------------------------------------

\subsection{Proof of Proposition~\ref{propo:potential}}
\label{sec:appen_smooth_proof}

From \eqref{eq:grad_cost} for any $\flow \in \flows$, we have:
%
\begin{align}
& \norm{\nabla \cost \parens{\flow} -  \nabla \cost \parens{\flowalt}}_{\infty} \nonumber \\
%
= &  \max_{\pair \in \pairs \atop \route \in \routes_\pair}  \abs*{\ex \bracks*{\sum_{\edge \in \route}  \late_{\edge} \parens*{\load_{\edge}(\flow), \sample} } - \ex \bracks*{\sum_{\edge \in \route}  \late_{\edge} \parens*{\load_{\edge}(\flowalt), \sample} } } \nonumber\\
%
\le & \max_{\pair \in \pairs \atop \route \in \routes_\pair} \ex \bracks*{ \abs*{ \sum_{\edge \in \route} \late_{\edge} \parens*{\load_{\edge}(\flow), \sample } -  \late_{\edge} \parens*{ \load_{\edge}(\flowalt), \sample }}}  \nonumber\\
%
\le & \max_{\pair \in \pairs \atop \route \in \routes_\pair} \ex \bracks*{ \sum_{\edge \in \route} \lips \abs*{  \load_{\edge}(\flow) -   \load_{\edge}(\flowalt) }}  \tag*{(due to Assumption~\ref{assum:blanket})} \nonumber\\
%
\le & \max_{\pair \in \pairs \atop \route \in \routes_\pair} \ex \bracks*{ \lips  \sum_{\edge \in \route}  \sum_{\pairalt \in \pairs} \sum_{\routealt \in \routes_\pairalt \atop \routealt \ni \edge} \abs*{\flow_{\pairalt,\routealt} - \flowalt_{\pairalt,\routealt} }}  \nonumber\\
%
\le & \ex \bracks*{ \lips  \sum_{\edge \in \edges}  \sum_{\pairalt \in \pairs} \sum_{\routealt \in \routes_\pairalt \atop \routealt \ni \edge} \abs*{\flow_{\pairalt,\routealt} - \flowalt_{\pairalt,\routealt} }} . \label{eq:proof_bderiv}
\end{align}
%

Now, for any $\pair \in \pairs$, we denote the length  a path $\route \in \routes_\pair$ by $\length_\route$ (\ie the number of edges containing in $\route$). Recall that $\length$ denotes the length of the longest paths in $\routes =\bigcup_{\pair \in \pairs} \routes_\pair$, we have
%
\begin{align*}
\sum_{\pairalt \in \pairs} \sum_{\routealt \in \routes_\pairalt} \abs*{ \flow_{\pairalt, \routealt} - \flowalt_{\pairalt, \routealt}} & =  \sum_{\pairalt \in \pairs} \sum_{\routealt \in \routes_\pairalt} \sum_{\edge \in \routealt}\frac{\abs*{  \flow_{\pairalt, \routealt} - \flowalt_{\pairalt, \routealt}}}{\length_\routealt}
%
\ge  \sum_{\pairalt \in \pairs} \sum_{\routealt \in \routes_\pairalt} \sum_{\edge \in \routealt}\frac{\abs*{  \flow_{\pairalt, \routealt} - \flowalt_{\pairalt, \routealt}}}{\length}
%
= \frac{1}{\length} \sum_{\edge \in \edges} \sum_{\pairalt \in \pairs}   \sum_{\routealt \in \routes_\pairalt \atop \routealt \ni \edge} {\abs*{\flow_{\pairalt, \routealt}   -  \flowalt_{\pairalt, \routealt}}}. 
\end{align*}

Combine this with \eqref{eq:proof_bderiv}, we have \mbox{$\norm{\nabla \cost \parens*{\flow} - \nabla \cost \parens*{\flowalt}}_{\infty}  \le  \length \lips \sum\limits_{\pairalt \in \pairs} \sum \limits_{\routealt \in \routes_\pair} \abs*{ \flow_{\pairalt, \routealt} - \flowalt_{\pairalt, \routealt}} = \norm{\flow - \flowalt}_1$}. This shows that $\cost$ is a $\smooth$-smooth function where $\smooth:= \length \lips$ and we conclude the proof of this~proposition.
\qed


















%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%--------------------------------------------------------
%-----------------------------------------------------------
\subsection{Proof of Theorem~\ref{theo:acceleweight}}
Theorem~\ref{theo:acceleweight} considers the stationary regime where we fix a parameter vector $\sample \in \samples$. In this setting, from~\eqref{eq:grad_cost}, we also have $\grad \cost(\flow) = \Late (\flow, \sample)$ for any flow $\flow \in \flows$. Due to this reason, in this section, we will use recurrently the exchange of these notations without further explanation. 

We will prove this theorem in the following 4 steps. 

\textit{\underline{Step 1:} Justify that $\flow^{\run} \in \flows$, $\forall \run$}. Indeed, by its definition in Line~\ref{line:AcceEW_ppoint}-Algorithm~\ref{algo:AccExpGrad},  we have $\ppoint^{\run} \in \flows, \forall \run$. Moreover, due to the choice of $\step^{\beforestart}$, we trivially have that $\flow^{\start} = \ppoint^{\start} \in \flows$. Now, for any $\run >1$, assume that $\flow^{\run-1} \in \flows$; therefore, \mbox{$\flow^{\run} = \step^{\run-1} \flow^{\run-1} + (1- \step^{\run-1}) \ppoint^{\run}$} also belongs to $\flows$ (since $\flows$ is a convex set). By proof of induction, we have that $\flow^{\run} \in \flows, \forall \run$.








%Use the regularizer $\hreg$ defined above and 
%recall that in the stationary setting in consideration, the notation $\lateest_{\edge} (\cdot)$ used in Algorithm~\ref{algo:AccExpGrad} is defined such that \mbox{$\sum_{\edge \in \route} \rat_\pair \lateest_{\edge}(\ppointalt^{\run}, \rat) =  \sum_{\edge \in \route} {\rat_\pair  {\late_{\edge} \parens*{\sum_{\pair \in \pairs} \rat_{\pair} \ppointalt^{\run}_{\edge} }}} = \nabla_{\pair, \route} \cost (\ppointalt^{\run})$} for any $\run$, we can rewrite Line~\ref{line:AcceEW_ppoint} of Algorithm~\ref{algo:AccExpGrad} as follows:\footnote{We prove this by defining $\obj\parens*{\ppoint, \lambda} = \parens{1 \!-\! \step^{\run\!-\!1}}   \stepalt^{\run\!-\!1}  \inner{\nabla \cost \parens{\ppointalt^{\run-1}}}{\ppoint \!-\! \ppoint^{\run-1} }  \!+\!    \dkl{\ppoint}{\ppoint^{\run-1} } \!-\! \sum_{\pair \in \pairs}\lambda_{\pair} \cdot \parens*{\sum_{\route \in \routes_\pair} \ppoint_{\pair, \route}\!-\!1}$ where \mbox{$\lambda = \parens*{\lambda_\pair}_{\pair \in \pairs} \in \mathbb{R}^{\nPairs}$} are the Lagrange multipliers corresponding to the constraints (\wrt to O-D pair $\pair$) of the set $\flows$. Then, we consider the system $\frac{\partial \obj}{\partial \ppoint_{\pair, \route}} \parens*{\ppoint, \lambda} =0$, $\frac{\partial \obj}{\partial \lambda_\pair} \parens*{\ppoint, \lambda} =0$, $\forall \pair \in \pairs, \forall \route \in \routes_\pair$. We can see that $\ppoint_{\pair, \route} =   \frac{\ppoint^{\run-1}_{\pair, \route} \exp \parens*{ -\parens{1- \step^{\run-1}} \stepalt^{\run-1} \nabla_{\pair, \route} \cost \parens*{\ppointalt^{\run-1}}} }    { \sum \limits_{\routealt \in \routes_\pair} \ppoint^{\run-1}_{\pair, \routealt} \exp \parens*{ -\parens{1- \step^{\run-1}} \stepalt^{\run-1}  \nabla_{\pair, \routealt} \cost \parens*{\ppointalt^{\run-1}}} } $, $\forall \pair \in \pairs$, $\forall \route \in \routes_\pair$ and \mbox{$\lambda_\pair =  \sum \limits_{\routealt \in \routes_\pair} \ppoint^{\run-1}_{\pair, \routealt} \exp \parens*{ -\parens{1- \step^{\run-1}} \stepalt^{\run-1}  \nabla_{\pair, \routealt} \cost \parens*{\ppointalt^{\run-1}}}$}, $\forall \pair \in \pairs$ is a solution of this system.}
%%
%\begin{equation}
%\ppoint^{\run} = \argmin \limits_{\ppoint \in \flows} \braces*{\parens{1- \step^{\run-1}}   \stepalt^{\run-1}  \inner{\nabla \cost \parens{\ppointalt^{\run-1}}}{\ppoint - \ppoint^{\run-1} }  +    \dkl{\ppoint}{\ppoint^{\run-1}  } }.  \label{eq:AcceEW_generalized_dpointalt} 
%\end{equation}



\textit{\underline{Step 2:} Define \mbox{$\Delta^{\run} := \stepalt^{\run - 1} \bracks*{\cost \parens{\flow^\run} - \cost \parens{\flowbase}} + \dkl{\flowbase}{\ppoint^\run }$} and prove that $\Delta^\run$ is a decreasing sequence as $\run$~increases.} Here, $\flow^\run, \ppoint^\run, \stepalt^{\run - 1}$ are defined as in Algorithm~\ref{algo:AccExpGrad} and $\flowbase$ is any equilibrium of the~game.

Fix an iteration $\run \ge \start$. Since $\cost$ is a $\smooth$-smooth function on $\flows$ \wrt the $\norm{\cdot}_1$ norm (cf. Proposition~\ref{propo:potential}), we have:
%
\begin{align}
	& \dis \cost\parens*{\flow^{\run + 1}} \nonumber\\
	%
	\le & \cost \parens*{\ppointalt^\run} + \inner{\nabla \cost \parens{\ppointalt^\run } }{\flow^{\run+1} - \ppointalt^\run} + \frac{\smooth}{2} \norm{\flow^{\run+1} - \ppointalt^\run}_1^2 \tag*{(due to \eqref{eq:smooth-alter})} \nonumber \\
%
	= &  \cost \parens*{\ppointalt^\run} + \inner{\nabla \cost \parens{\ppointalt^\run } }{\flow^{\run+1} - \ppointalt^\run} +  \frac{\smooth}{2} \parens*{ 1 - \step^\run}^2 \norm{\ppoint^{\run + 1} - \ppoint^\run}_1^2  \tag*{(from Lines~\ref{line:AcceEW_flow} and \ref{line:AcceEW_dpoint} of Algorithm~\ref{algo:AccExpGrad})} \nonumber \\
%
	\le & \cost \parens*{\ppointalt^\run} + \inner{\nabla \cost \parens{\ppointalt^\run } }{\flow^{\run+1} - \ppointalt^\run} +  \frac{\smooth}{2} \parens*{ 1 - \step^\run}^2 \cdot 2 \massmax \nPairs \cdot \dkl{\ppoint^{\run + 1}}{\ppoint^\run}  \tag*{(since $\hreg$ is $\frac{1}{\massmax \nPairs }$-strongly convex)} \nonumber \\
%
	= & \cost \parens*{\ppointalt^\run} + \inner{\nabla \cost \parens{\ppointalt^\run } }{\flow^{\run+1} - \ppointalt^\run} +  {\smooth\massmax \nPairs} \parens*{ 1 - \step^\run}^2  \dkl{\ppoint^{\run + 1}}{\ppoint^\run}.   \label{eq:apply_lem_smoothdef}
\end{align}







On the other hand, from the convexity of $\cost$, we have
\begin{align}
	\step^\run \cost \parens*{\flow^\run } + \parens*{1 - \step^\run } \cost \parens*{\flowbase} \ge \cost \parens*{\step^\run \flow^\run + \parens*{1- \step^\run} \flowbase } \ge  \cost\parens*{ \ppointalt^\run} + \inner{\grad \cost\parens*{ \ppointalt^\run}}{ \step^\run \flow^\run + \parens*{1- \step^\run} \flowbase - \ppointalt^\run}, \nonumber
\end{align}
which deduces the following inequality:
%
\begin{align}
	&\cost\parens*{\flow^{\run + 1}} -  \cost\parens*{\flowbase} - \step^\run \bracks{ \cost\parens*{\flow^{\run}} -  \cost\parens*{\flowbase} }   \nonumber \\
	%
	= & \cost\parens*{\flow^{\run + 1}} - \bracks{\step^\run \cost\parens*{\flow^\run} + \parens{1 -\step^\run}  \cost\parens*{\flowbase}}   \nonumber \\
	%
	\le &  \cost\parens*{\flow^{\run + 1}} -  \cost\parens*{\ppointalt^{\run}} + \inner{\nabla  \cost\parens*{\ppointalt^{\run}}}{ \ppointalt^\run - \step^\run \flow^\run - \parens*{1- \step^\run} \flowbase}   \nonumber\\
	%
	\le &  \inner{\nabla \cost \parens{\ppointalt^\run } }{\flow^{\run+1} - \ppointalt^\run} +     \smooth \massmax \nPairs \parens*{ 1 - \step^\run}^2 \dkl{\ppoint^{\run + 1}}{\ppoint^\run} + \inner{\nabla  \cost\parens*{\ppointalt^{\run}}}{ \ppointalt^\run - \step^\run \flow^\run - \parens*{1- \step^\run} \flowbase} \tag*{(due to \eqref{eq:apply_lem_smoothdef})} \nonumber \\
	%
	= & \inner{\nabla  \cost\parens*{\ppointalt^{\run}}}{ \flow^{\run+1} - \step^\run \flow^\run - \parens*{1- \step^\run} \flowbase}  +    \smooth \massmax \nPairs \parens*{ 1 - \step^\run}^2 \dkl{\ppoint^{\run + 1}}{\ppoint^\run}  \nonumber \\
	%
	= & \parens*{1 - \step^\run}  \inner{\nabla  \cost\parens*{\ppointalt^{\run}}}{ \ppoint^{\run+1} - \flowbase} + \smooth \massmax \nPairs \parens*{ 1 - \step^\run}^2 \dkl {\ppoint^{\run + 1}}{\ppoint^\run}.\label{eq:proof_AMC_inequ_proof_1}
	%
\end{align}
%
Here, the last equality comes from Line \ref{line:AcceEW_flow} of Algorithm~\ref{algo:AccExpGrad}. Multiplying two sides of \eqref{eq:proof_AMC_inequ_proof_1} by $\stepalt^\run$, we have
%
\begin{align}
	\stepalt^\run \bracks{ \cost\parens*{ \flow^{\run + 1}} -  \cost\parens*{ \flowbase} } -  \stepalt^\run \step^\run \bracks{ \cost\parens*{ \flow^{\run}} -  \cost\parens*{ \flowbase} } \le & \parens*{1 - \step^\run}  \stepalt^\run  \inner{\nabla  \cost\parens*{\ppointalt^{\run}}}{ \ppoint^{\run+1} -  \flowbase} + \stepalt^\run   \smooth \massmax \nPairs\parens*{ 1 - \step^\run}^2 \dkl{\ppoint^{\run + 1}}{\ppoint^\run}.\label{eq:proof_AMC_1}
\end{align}
%


Now, for the sake of brevity, let us denote \mbox{$\dpointalt^{\run} =  \parens{1- \step^{\run}}   \stepalt^{\run} \Late(\ppointalt^{\run}, \sample) =  \parens{1- \step^{\run}}   \stepalt^{\run} \nabla \cost(\ppointalt^{\run})$} for any $\pair \in \pairs$ and $\route \in \routes_\pair$. From the facts that $\ppoint^{\run+1} = \logit \parens*{\dpoint^{\run}}$ (see Line~\ref{line:AcceEW_ppoint} of Algorithm~\ref{algo:AccExpGrad}) and that \mbox{$\dpoint^{\run} = \sum_{\runalt =1 }^{\run} \dpointalt^{\runalt}$} (see Line~\ref{line:AcceEW_dpoint} of Algorithm~\ref{algo:AccExpGrad}), we can rewrite that \mbox{$\ppoint^{\run+1}_{\pair, \route}= \mass_{\pair} \frac{\ppoint^{\run}_{\pair, \route} \exp ( -\dpointalt^{\run}_{\route} )}{\sum_{\routealt \in \routes_\pair} \ppoint^{\run}_{\pair, \routealt} \exp(-\dpointalt^{\run}_{\routealt})}$}. Therefore, we have:
\begin{align}
	& \inner{\nabla \hreg(\ppoint^{\run}) - \nabla \hreg(\ppoint^{\run+1})}{ \ppoint^{\run+1} - \flowbase } \nonumber\\
	%
	= &	\sum_{\pair \in \pairs} \sum_{\route \in \routes} \log \parens*{ \frac{\ppoint^{\run}_{\pair, \route}}{\ppoint^{\run+1}_{\pair, \route}} } \parens*{\ppoint^{\run+1}_{\pair, \route} - \flowbase_{\pair, \route} } \nonumber\\
	%
	= & \sum_{\pair \in \pairs} \sum_{\route \in \routes} \log \parens*{ \frac{\ppoint^{\run}_{\pair, \route}}{\mass_{\pair} \frac{\ppoint^{\run}_{\pair, \route} \exp ( -\dpointalt^{\run}_{\route} )}{\sum_{\routealt \in \routes_\pair} \ppoint^{\run}_{\pair, \routealt} \exp(-\dpointalt^{\run}_{\routealt})}} } \parens*{\ppoint^{\run+1}_{\pair, \route} - \flowbase_{\pair, \route} } \nonumber\\
	%
	=& \sum_{\pair \in \pairs} \sum_{\route \in \routes} \log \parens*{ \frac{\sum_{\routealt \in \routes_\pair} \ppoint^{\run}_{\pair, \routealt} \exp(-\dpointalt^{\run}_{\routealt}) }{ \mass_{\pair} } } \parens*{\ppoint^{\run+1}_{\pair, \route} - \flowbase_{\pair, \route} }  - 	\sum_{\pair \in \pairs} \sum_{\route \in \routes} \log \parens*{ \exp( -\dpointalt^{\run}_{\pair, \route}) } \parens*{\ppoint^{\run+1}_{\pair, \route} - \flowbase_{\pair, \route} } \nonumber\\
	%
	=& \sum_{\pair \in \pairs} \log \parens*{ \frac{\sum_{\routealt \in \routes_\pair} \ppoint^{\run}_{\pair, \routealt} \exp(-\dpointalt^{\run}_{\routealt}) }{ \mass_{\pair} } }  \sum_{\route \in \routes_\pair} \parens*{\ppoint^{\run+1}_{\pair, \route} - \flowbase_{\pair, \route} }  + \sum_{\pair \in \pairs} \sum_{\route \in \routes} \dpointalt^{\run}_{\pair,\route} \parens*{\ppoint^{\run+1}_{\pair, \route} - \flowbase_{\pair, \route} } \nonumber\\
	%
	=& 0 + \inner{\dpointalt^{\run}}{ \ppoint^{\run+1} - \flowbase} \tag*{(since $ \sum_{\route \in \routes_{\pair}} \ppoint^{\run+1}_{\pair, \route} =\sum_{\route \in \routes_{\pair}} \flowbase_{\pair, \route} = \mass_{\pair}, \forall \pair \in \pairs$)} \nonumber\\
	%
	=&  \parens{1- \step^{\run}}   \stepalt^{\run}  \inner{ \nabla \cost (\ppointalt^{\run})}{ \ppoint^{\run+1} - \flowbase}. \label{eq:app_acceleweight_equality}
\end{align}

Combining \eqref{eq:app_acceleweight_equality} with \eqref{eq:proof_AMC_1}, then apply \eqref{eq:BregmanTriangle}, we obtain that:
\begin{align}
	& \stepalt^\run \bracks{ \cost\parens*{ \flow^{\run + 1}} -  \cost\parens*{ \flowbase} } -  \stepalt^\run \step^\run \bracks{ \cost\parens*{ \flow^{\run}} -  \cost\parens*{ \flowbase} } \nonumber \\
%
	\le &  \inner{ \nabla \hreg \parens*{\ppoint^\run} - \nabla \hreg \parens*{\ppoint^{\run+1}} }{ \ppoint^{\run+1} -  \flowbase} + \stepalt^\run   \nPairs \massmax \smooth \parens*{ 1 - \step^\run}^2 \dkl{\ppoint^{\run + 1}}{\ppoint^\run} \nonumber \\
%
	\le & \dkl{ \flowbase}{\ppoint^\run} - \dkl{ \flowbase}{\ppoint^{\run+1}} - \dkl{\ppoint^{\run+1}}{\ppoint^\run} + \stepalt^\run   \nPairs \massmax \smooth \parens*{ 1 - \step^\run}^2 \dkl{\ppoint^{\run + 1}}{\ppoint^\run} \nonumber \\
%
	= & \dkl{ \flowbase}{\ppoint^\run} - \dkl{ \flowbase}{\ppoint^{\run+1}} + \parens*{\stepalt^\run   \nPairs \massmax \smooth \parens*{ 1 - \step^\run}^2 - 1} \dkl{\ppoint^{\run + 1}}{\ppoint^\run}. \label{eq:proof_AMD_conclu}
\end{align}



From the update rule of $\stepalt^{\run}$ in Line \ref{line:AcceEW_stepalt}, the choice of $\stepalt^{0}$ in Line \ref{line:AcceEW_initial} and the update rule of $\step^{\run}$ in Line~\ref{line:AcceEW_step}, we can trivially obtain that
\begin{equation}
	\stepalt^\run  \nPairs \massmax \smooth \parens*{ 1 - \step^\run}^2 =  	\stepalt^\run \frac{1}{\stepalt^{\beforestart}} \parens*{ 1 - \frac{\stepalt^{\run-1}}{\stepalt^{\run}}}^2 =  \frac{ \parens*{\stepalt^{\run-1} - \stepalt^{\run}}^2 }{\stepalt^\run \stepalt^{\beforestart} } = 1. \label{eq:app_acceleweight_stepaltcompute}
\end{equation}
%
Therefore, the last term in \eqref{eq:proof_AMD_conclu} equals zero and we can rewrite \eqref{eq:proof_AMD_conclu} as: 
\begin{equation*}
	\stepalt^{\run} \bracks*{\cost \parens{ \flow^{\run + 1}} - \cost \parens{ \flowbase}} + \dkl{ \flowbase}{\ppoint^{\run+1} }  \le  \stepalt^{\run - 1} \bracks*{\cost \parens{ \flow^\run} - \cost \parens{ \flowbase}} + \dkl{ \flowbase}{\ppoint^\run } .
\end{equation*}
%
This shows precisely that $\Delta^\nRuns \le \Delta^{\nRuns-1} \le \ldots \le \Delta^{\beforestart}$ (by convention, we set $\stepalt^{-1} =0$). Particularly, we have:
\begin{equation}
	\stepalt^{\nRuns-1} \bracks*{\cost \parens{ \flow^{\nRuns}} - \cost \parens{ \flowbase}} \le \stepalt^{\nRuns-1} \bracks*{\cost \parens{ \flow^{\nRuns}} - \cost \parens{ \flowbase}} + \dkl{ \flowbase}{\ppoint^{\nRuns} }  := \Delta^{\nRuns} \le \Delta^{\nRuns-1} \le \ldots \le \Delta^{\start} = \dkl{ \flowbase}{\ppoint^{\beforestart} }.\label{eq:proof_AMC_last}
\end{equation}
% %
%
%%
%
%
\textit{\underline{Step 3:} Prove the following inequality for any equilibrium flow $\flowbase$ of the mean game $\mgame$ and the output $\flow^{\nRuns}$ of Algorithm~\ref{algo:AccExpGrad} at any arbitrary time $\nRuns>0$:}
\begin{equation}
	\cost\parens*{ \flow^\nRuns} - \cost\parens{ \flowbase} \le \frac{ 4   \smooth \dkl{ \flowbase}{\ppoint^{\start}} }{\parens{\nRuns - \afterstart}^2}= \frac{ 4   \smooth\dkl{\flowbase}{\flow^{\start}} }{\parens{\nRuns - \afterstart}^2 }. \label{eq:AcceEW_generalized_regret}
\end{equation}


To prove \eqref{eq:AcceEW_generalized_regret}, we first look for a lower-bound of $\stepalt^{\nRuns-1}$. From \eqref{eq:app_acceleweight_stepaltcompute}, we have
\begin{equation}
	\sqrt{ \stepalt^{\run-1}\nPairs \massmax \smooth } =  \sqrt{   \stepalt^{\run} \nPairs \massmax \smooth} \sqrt{1- \frac{1}{ \sqrt{ \stepalt^{\run} \nPairs \massmax \smooth } }} \label{eq:proof_AMC_bound_gamma}.
\end{equation}

Now, consider the function $l\parens{\real}: (0,1] \rightarrow \Rpos$ such that $l \parens{\real} = \parens*{1-\real}^{1/2}, \forall \real \in (0,1]$. Note that, from Line \ref{line:AcceEW_stepalt} of Algorithm~\ref{algo:AccExpGrad}, $\stepalt^\run$ is an increasing sequence and thus, for any $\run \ge 1$, $\stepalt^{\run} \ge \stepalt^{\beforestart} = 1/\parens*{  \nPairs \massmax \smooth}$ which implies that $0< \frac{1}{\sqrt{  \nPairs \massmax \smooth \stepalt^{\run}}} \le 1 $. From the fact that $l$ is a concave function, we have:
\begin{align*}
	& l \parens*{\frac{1}{\sqrt{ \nPairs \massmax \smooth \stepalt^{\run}}}} \le   l \parens*{0} -  l^{\prime}\parens{0}\parens*{\frac{1}{\sqrt{ \nPairs \massmax \smooth \stepalt^{\run}}} -0 } \\
	%
	\Rightarrow & \parens*{1 - \frac{1}{\sqrt{ \nPairs \massmax \smooth \stepalt^{\run}}} }^{1/2} \le 1 - \frac{1}{2 \sqrt{   \nPairs \massmax \smooth \stepalt^{\run}} }
\end{align*}
%   
Combining this with \eqref{eq:proof_AMC_bound_gamma}, we obtain $\sqrt{ \nPairs \massmax \smooth \stepalt^{\run}} \ge \sqrt{ \nPairs \massmax \smooth \stepalt^{\run}} + 1/2$. Therefore, 
\begin{align*}
	\sqrt{\nPairs \massmax \smooth \stepalt^{\nRuns-1}} \ge   \sqrt{  \nPairs \massmax \smooth \stepalt^{\nRuns-2}}  + \frac{1}{2} \ge \ldots \ge    \sqrt{ \nPairs \massmax \smooth \stepalt^{\beforestart}}  + \frac{\nRuns-\start}{2} = \frac{\nRuns-\start}{2}. 
\end{align*}
%
This implies that $ \stepalt^{\nRuns-1}  > \frac{\parens*{\nRuns -\start}^2}{4  \nPairs \massmax \smooth} >0$; combining this with \eqref{eq:proof_AMC_last}, we have 
\begin{equation*}
	\cost\parens*{ \flow^\nRuns} - \cost\parens{ \flowbase} \le \frac{ 4  \nPairs \massmax \smooth \dkl{ \flowbase}{\ppoint^{\start}} }{\parens{\nRuns - \start}^2}= \frac{ 4\nPairs \massmax \smooth \dkl{ \flowbase}{ \flow^{\start}} }{\parens{\nRuns - \start}^2 }.
\end{equation*}
We finish the proof of \eqref{eq:AcceEW_generalized_regret} here.







\textit{\underline{Step 4:} Upper-bound $\cost\parens*{\flow^{\nRuns}} - \cost \parens*{\flowbase}$ to find the convergence rate.}

To do this, we only need to find an upper-bound of $\dkl{\flowbase}{\flow^{\start}}$ then apply~\eqref{eq:AcceEW_generalized_regret}. First, from the choice of $\dpoint^{\beforestart}$ and $\step^{\beforestart}$ in Line~\ref{line:AcceEW_initial} of Algorithm~\ref{algo:AccExpGrad}, we have $\flow^{\start}_{\pair, \route} = \ppoint^{\start}_{\pair, \route} = \mass_{\pair} \big/ \nRoutes_\pair$ for any $\pair\in \pairs$ and $\route \in \routes_\pair$; therefore, we have
\begin{align}
	&\inner{\nabla \hreg \parens{\flow^{\start}}}{\flow^{\start}-\flowbase}  \nonumber \\
	%
	= &  {\sum_{\pair \in \pairs} \sum_{\route \in \routes_\pair} \log \parens*{\flow^{\start}_{\pair, \route}} \flow^{\start}_{\pair, \route} +  \sum_{\pair \in \pairs} \sum_{\route \in \routes_\pair} \flow^{\start}_{\pair, \route}  +    \sum_{\pair \in \pairs} \sum_{\route \in \routes_\pair} \log \parens*{\flow^{\start}_{\pair, \route}} \flowbase_{\pair, \route} +  \sum_{\pair \in \pairs} \sum_{\route \in \routes_\pair} \flowbase_{\pair, \route} }   \nonumber\\
	%
	= &  { \sum_{\pair \in \pairs} \sum_{\route \in \routes_\pair} \frac{\mass_{\pair} \log \parens*{\mass_{\pair} \big/ \nRoutes_\pair} }{\nRoutes_\pair }  +  \sum_{\pair \in \pairs} \sum_{\route \in \routes_\pair} \frac{\mass_{\pair}}{\nRoutes_\pair} + \sum_{\pair \in \pairs} \sum_{\route \in \routes_\pair} \log \parens*{\mass_{\pair} \big/ \nRoutes_\pair } \flowbase_{\pair, \route}  +  \sum_{\pair \in \pairs} \sum_{\route \in \routes_\pair} \flowbase_{\pair, \route}}  \nonumber\\
	%
	=&  2 \sum_{\pair \in \pairs} \mass_{\pair} \log \parens*{\mass_{\pair} \big/ \nRoutes_\pair}  +  2 \sum_{\pair \in \pairs} \mass_{\pair}  \tag*{(since $\sum_{\route \in \routes_\pair} \flowbase_{\pair, \route} =\mass_{\pair}, \forall \pair \in \pairs$)} \nonumber\\
	%
	\le & 2 \sum_{\pair \in \pairs} \mass_{\pair} \log \parens*{\mass_{\pair} } - 2 \sum_{\pair \in \pairs} \mass_{\pair} \log \parens*{\nRoutes_\pair } +  2 \masssum \nonumber\\
	%
	\le & 2 \masssum \bracks*{\log(\massmax)+1}  \label{eq:app_acceleweight_end}
\end{align}
%

Now, by definition, we also have:
\begin{align}
	&\dkl{\flowbase}{\flow^{\start}} \nonumber\\
		%
	= & \hreg \parens*{\flowbase} -  \hreg \parens*{\flow^{\start}} - \inner{\nabla \hreg \parens{\flow^{\start}}}{\flowbase - \flow^{\start}} \nonumber\\
		 %
	\le  & -  \min_{\flow \in \flows}\hreg \parens*{\flow} +  \inner{\nabla \hreg \parens{\flow^{\start}}}{\flow^{\start} - \flowbase } \nonumber\\
		%
	\le &  \masssum \log(\nRoutes/\masssum) + 2 \masssum \bracks*{\log(\massmax)+1} \tag*{(from \eqref{eq:app_expweights_1st} and \eqref{eq:app_acceleweight_end})} \nonumber\\
	%
	= & \masssum \bracks*{ \log\parens*{\frac{\nRoutes \massmax^2}{\masssum}}  + 2}  \label{eq:proof_AccExpGrad_0}
%
\end{align}

Combine \eqref{eq:proof_AccExpGrad_0} and \eqref{eq:AcceEW_generalized_regret}, we obtain that

\begin{equation*}
\cost\parens*{\flow^\nRuns} - \cost\parens*{\flowbase} \le \frac{4 \nPairs \masssum  \massmax \smooth   \bracks*{ \log\parens*{\frac{\nRoutes \massmax^2}{\masssum}}  + 2}  }{\parens*{\nRuns-\start}^2}.
\end{equation*}
%
%%
This concludes the proof. \qed










==> App-expweights.tex <==
%----------------------------------------------------------------------
%%% APP: GAMEFORM
%----------------------------------------------------------------------
% !TEX root = ./Main.tex


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%---------------------------------
\subsection{Proof of Theorem~\ref{theo:expweights}}


%

Let $\hreg$ be the entropy regularizer defined in~\eqref{eq:entropy} and $\flowbase$ be any equilibrium flow of the mean game $\mgame$, we have:
\begin{align}
	& \mass \log(\massmax) + \sum_{\run = 1}^{\nRuns} \stepalt^{\run} \inner{\flowbase}{\Late(\flow^{\run}, \sample^{\run})}   \\
	%
	  = & \sum_{\pair \in \pairs} \sum_{\route \in \routes_{\pair}} \flowbase_{\pair,\route} \log(\massmax) +  \sum_{\run = 1}^{\nRuns} \stepalt^{\run} \inner{\flowbase}{\Late(\flow^{\run}, \sample^{\run})}   \nonumber\\
	 %
	 = &  \sum_{\pair \in \pairs} \sum_{\route \in \routes_{\pair}} \flowbase_{\pair,\route} \log(\flowbase_{\pair, \route}) -  \sum_{\pair \in \pairs} \sum_{\route \in \routes_{\pair}} \flowbase_{\pair,\route} \log\parens*{ \frac{\flowbase_{\pair,\route}}{\massmax}}   + \sum_{\run = 1}^{\nRuns} \stepalt^{\run} \inner{\flowbase}{\Late(\flow^{\run}, \sample^{\run})} \nonumber\\
	 %
	\ge  & \hreg(\flowbase) + \sum_{\run = 1}^{\nRuns} \stepalt^{\run} \inner{\flowbase}{\Late(\flow^{\run}, \sample^{\run})}  \qquad \qquad \tag*{\textrm{(since } $\log\parens*{\frac{\flowbase_{\pair, \route}}{\massmax}} \le 0, \forall \pair \in \pairs, \forall \route \in \routes_\pair$ \textrm{)}}	 \nonumber\\
	 %
	   = &	\hreg(\flowbase) - \inner*{\flowbase}{-\sum_{\run =1}^{\nRuns} \stepalt^{\run} \Late(\flow^{\run}, \sample^{\run})} \nonumber\\
	%
	 = & \hreg(\flowbase) - \inner*{\flowbase}{\dpoint^{\nRuns}} \tag*{ \textrm{(due to Line~\ref{line:EW_dpoint} of Algorithm~\ref{algo:expweights})} }\nonumber \\
	%
	  \ge& - \hreg^{\ast} ( \dpoint^{\nRuns}) \tag*{\textrm{(due to Fenchel-Young inequality)}} \nonumber\\
	%
		 = & - \hreg^{\ast} (\dpoint^{0}) - \sum_{\run=1}^{\nRuns} \bracks*{ \hreg^{\ast} (\dpoint^{\run}) - \hreg^{\ast} (\dpoint^{\run-1})} \nonumber\\
	 %
	 	 = & - \hreg^{\ast} (\dpoint^{0}) -  \sum_{\run=1}^{\nRuns}\sum_{\pair \in \pairs} \mass_{\pair} \log \parens*{\frac{\sum_{\route \in \routes_\pair}\exp\parens*{  \dpoint_{\pair,\route}^{\run}}}{\sum_{\routealt \in \routes_\pair}\exp\parens*{ \dpoint_{\pair, \routealt}^{\run-1}}}} \tag*{\textrm{(by definition of} $\hreg^{\ast}$ \textrm{)}} \nonumber\\
 	%
 		 = & - \hreg^{\ast} (\dpoint^{0}) -  \sum_{\run=1}^{\nRuns} \sum_{\pair \in \pairs} \mass_{\pair} \log \parens*{ \frac{ \mass_{\pair}\sum_{\route \in \routes_\pair}\exp\parens*{  \dpoint_{\pair,\route}^{\run-1}} \exp\parens*{ - \stepalt^{\run} \late_{\route}(\flow^{\run}, \sample^{\run})  } }{  \sum_{\routealt \in \routes_\pair}\exp\parens*{ \dpoint_{\pair, \routealt}^{\run-1}}} \cdot \frac{1}{\mass_{\pair}}}  \nonumber\\
 		%
 		& = - \hreg^{\ast} (\dpoint^{0}) -  \sum_{\run=1}^{\nRuns} \bracks*{ \sum_{\pair \in \pairs} \mass_{\pair}  \log \parens*{  \sum_{\route \in \routes_\pair} \flow^{\run}_{\pair, \route} \exp\parens*{ - \stepalt^{\run} \late_{\route}(\flow^{\run}, \sample^{\run})  }  } - \sum_{\pair \in \pairs} \mass_{\pair}\log(\mass_\pair)}.\label{eq:app_expweight_start}
\end{align}
%
We will find the lower bounds of the terms in the right-hand-size of \eqref{eq:app_expweight_start}. First, since we chose $\dpoint^{0} = \boldsymbol{0}$, we have $\hreg^{\ast}(\dpoint^0) = \max_{\flow \in \flows} \parens*{\inner{\boldsymbol{0}}{\flow} -\hreg(\flow) } =  -\min_{\flow \in \flows} \hreg(\flow) =  \min\limits_{\flow \in \flows}   \sum \limits_{\pair \in \pairs} \sum\limits_{\route \in \routes_\pair} \flow_{\pair, \route} \log \parens*{\frac{1}{\flow_{\route, \pair}}  }$. Moreover, apply Jensen's inequality on the function $\log(\cdot)$ (that is a concave function), for any $\flow \in \flows$, we have: \mbox{$ \sum \limits_{\pair \in \pairs} \sum\limits_{\route \in \routes_\pair} \flow_{\pair, \route} \log \parens*{\frac{1}{\flow_{\route, \pair}}  } \le \parens*{\sum \limits_{\pair \in \pairs} \sum\limits_{\route \in \routes_\pair}\flow_{\pair,\route} } \log \parens*{ \frac{ \sum \limits_{\pair \in \pairs} \sum\limits_{\route \in \routes_\pair} \frac{\flow_{\pair, \route}}{\flow_{\pair, \route}} }{ \sum\limits_{\pair \in \pairs} \sum\limits_{\route \in \routes_\pair} \flow_{\pair, \route}  } } = \masssum \log \parens*{\nRoutes / \masssum} $}. Therefore, 
\begin{equation}
	- \hreg^{\ast}(\dpoint^{0}) = \min_{\flow \in \flows} \hreg(\flow) \ge- \masssum \log(\nRoutes/\masssum). \label{eq:app_expweights_1st} 
\end{equation}
%
%
Second, by the inequality $\exp\parens{-\alpha}\leq 1-\alpha+\alpha^{2}$ for all $\alpha \geq 0$, the second term in \eqref{eq:app_expweight_start} is bounded as~follows:
%
\begin{align}
	&   \sum_{\pair \in \pairs} \mass_{\pair}  \log \parens*{  \sum_{\route \in \routes_\pair} \flow^{\run}_{\pair, \route} \exp\parens*{ - \stepalt^{\run} \late_{\route}(\flow^{\run}, \sample^{\run})  } } - \sum_{\pair \in \pairs} \mass_{\pair}\log(\mass_\pair)   \nonumber\\
	%
 	& \le \sum_{\pair \in \pairs} \mass_\pair \log \parens*{  \sum_{\route \in \routes_\pair} \flow^{\run}_{\pair, \route} \parens*{1 -  \stepalt^{\run} \late_{\route}(\flow^{\run}, \sample^{\run})  + (\stepalt^{\run} \late_{\route}(\flow^{\run}, \sample^{\run}))^2 } }   - \sum_{\pair \in \pairs} \mass_{\pair}\log(\mass_\pair)   \nonumber  \\
	%
	&\le\sum_{\pair \in \pairs} \mass_{\pair} \log \parens*{\mass_{\pair} - \sum_{\route \in \routes_\pair} \flow^{\run}_{\pair, \route} \parens*{  \stepalt^{\run} \late_{\route}(\flow^{\run}, \sample^{\run})  - (\stepalt^{\run} \late_{\route}(\flow^{\run}, \sample^{\run}))^2 } }  - \sum_{\pair \in \pairs} \mass_{\pair}\log(\mass_\pair)   \nonumber \\
	%
	& \le \sum_{\pair \in \pairs} \mass_{\pair}  \log \parens*{\mass_\pair } + \sum_{\pair \in \pairs} \mass_{\pair} \log \parens*{  1 - \frac{ \sum_{\route \in \routes_\pair} \flow^{\run}_{\pair, \route} \parens*{  \stepalt^{\run} \late_{\route}(\flow^{\run}, \sample^{\run})  - (\stepalt^{\run} \late_{\route}(\flow^{\run}, \sample^{\run}))^2 }}{\mass_{\pair}} }   - \sum_{\pair \in \pairs} \mass_{\pair}\log(\mass_\pair) \nonumber\\
	%
	& \le  - \sum_{\pair \in \pairs}   \sum_{\route \in \routes_\pair} \flow^{\run}_{\pair, \route} \parens*{  \stepalt^{\run} \late_{\route}(\flow^{\run}, \sample^{\run})  - (\stepalt^{\run} \late_{\route}(\flow^{\run}, \sample^{\run}))^2 }  \label{eq:app_expweights_2ex}\\
	%
	&\le - \inner*{\flow^{\run}}{\stepalt^{\run} \Late (\flow^{\run}, \sample^{\run}) } +   \inner*{\flow^{\run}}{(\stepalt^{\run} \Late (\flow^{\run}, \sample^{\run}))^2 }  . \label{eq:app_expweights_2}
\end{align}
Here, \eqref{eq:app_expweights_2ex} comes from applying the inequality $\log(1-\alpha)\leq -\alpha$ for any $\alpha < 1$.

Now, combining \eqref{eq:app_expweights_1st} and \eqref{eq:app_expweights_2} with \eqref{eq:app_expweight_start}, we have 

\begin{align}
	  \sum_{\run = 1}^{\nRuns} \bracks*{ \inner*{\flow^{\run}}{\stepalt^{\run} \Late (\flow^{\run}, \sample^{\run}) } -  \inner{\flowbase}{\stepalt^{\run} \Late(\flow^{\run}, \sample^{\run})}}   \le  \masssum \log(\nRoutes \massmax/\masssum) + \sum_{\run = 1}^{\nRuns}    \inner*{\flow^{\run}}{(\stepalt^{\run} \Late (\flow^{\run}, \sample^{\run}))^2 } .\label{eq:app_expweights_conclude}
\end{align}
Now, from Assumption~\ref{assum:blanket}, \mbox{$\inner*{\flow^{\run}}{(\stepalt^{\run} \Late (\flow^{\run}, \sample^{\run}))^2  } =\dis  \sum_{\pair\in \pairs}\sum_{\route \in \routes_\pair}{\flow^{\run}_{\pair,\route} \bracks*{\stepalt^{\run} \late_{\route}(\flow^{\route}, \sample^{\run}) } }^2 \le  \sum_{\pair\in \pairs}\sum_{\route \in \routes_\pair}  \flow^{\run}_{\pair,\route} (\stepalt^{\run}\ub )^2 = (\stepalt^{\run}\ub )^2 \masssum$}. Therefore, from \eqref{eq:app_expweights_conclude} and by choosing $\stepalt^{\run} =1/\sqrt{\run}$, we have:
%
\begin{align}
		&\sum_{\run = 1}^{\nRuns} \stepalt^{\run} \inner*{\flow^{\run} - \flowbase}{ \Late(\flow^{\run}, \sample^{\run})}  \le \masssum \log(\nRoutes \massmax/\masssum) +  \mass \ub^2 \sum_{\run = 1}^{\nRuns} (\stepalt^{\run})^2 \nonumber\\
		%
		\Rightarrow & \sum_{\run = 1}^{\nRuns} \frac{1}{\sqrt{\run}} \inner*{\flow^{\run} - \flowbase}{ \Late(\flow^{\run}, \sample^{\run})}  \le \masssum \log(\nRoutes \massmax/\masssum) +  \mass \ub^2 \sum_{\run = 1}^{\nRuns} \frac{1}{\run} \nonumber\\
		%
	 	\Rightarrow & \sum_{\run = 1}^{\nRuns} \frac{1}{\sqrt{\nRuns}} \inner*{\flow^{\run} - \flowbase}{ \Late(\flow^{\run}, \sample^{\run})} \le  \masssum \log(\nRoutes \massmax/\masssum) +  \mass \ub^2 \parens*{\log(\nRuns) + 1} \nonumber\\
	 	%
 		\Rightarrow & \sum_{\run = 1}^{\nRuns} \inner*{\flow^{\run} - \flowbase}{ \Late(\flow^{\run}, \sample^{\run})} \le  \sqrt{\nRuns}\mass \log(\nRoutes \massmax/\mass) + \sqrt{\nRuns} \mass \ub^2 \parens*{\log(\nRuns) + 1}
\end{align} 
%
Now, from~\eqref{eq:grad_cost}, we have $\ex \bracks*{ \Late \parens*{\flow^{\run}, \sample^{\run}} } = \grad \cost (\flow^{\run})$ for any $\run = 1,2,\ldots$. Apply Theorem 4.1 of \cite{shalev2011online}, we~have:

%
\begin{align}
\ex \bracks*{\frac{1}{\nRuns} \sum_{\run=1}^{\nRuns}\cost (\flow^{\run}) - \cost(\flowbase) } =  \frac{1}{\nRuns}\ex\left[ \sum_{\run=1}^{\nRuns}\cost (\flow^{\run})-\cost (\flowbase)\right]  &   \leq   \frac{\masssum}{\sqrt{\nRuns}} \bracks*{   \log(\nRoutes \massmax/\masssum) +  \ub^2 \parens*{\log(\nRuns) + 1}}.\label{eq:app_expweights_end} 
\end{align}
%
Finally, since $\cost(\cdot)$ is a convex function on $\flows$, we have $\cost \parens*{ \frac{1}{\nRuns} \sum_{\run=1}^{\nRuns} \flow^{\run} } \le \frac{1}{\nRuns} \sum_{\run=1}^{\nRuns}\cost (\flow^{\run})$. Combining this with \eqref{eq:app_expweights_end}, we conclude the proof.\qed

%On the other hand, from \eqref{eq:grad_rosenthal}, for any $\run \in \bracks*{\nRuns}$, we have 
%\begin{equation}
%\norm{\nabla \cost \parens*{ \flow^\run} }_{\infty}:= \max \limits_{\pairbase \in \pairs \atop \routebase \in \pairbase} \braces*{ \nabla_{\pairbase, \routebase} \cost \parens*{\flow}} \!=\! \max \limits_{\pairbase \in \pairs \atop \routebase \in \pairbase} \braces*{\sum \limits_{\edge \in \routebase} \rat_\pairbase  {\late_{\edge} \parens*{\sum \limits_{\pair \in \pairs} \! \sum\limits_{\route \in \routes_\pair \atop \route \ni \edge} \rat_\pair \flow_{\pair, \route}}}} \le \ratmax^2 \length \ub:= \lips_0. \label{eq:maxnom_grad}
%\end{equation}


%Finally, combining \eqref{eq:basic_EW}, \eqref{eq:regular_entropy}, \eqref{eq:maxnom_grad}  and the fact that $\cost$ is a convex function,\footnote{By the definition of $\cost$ and the fact that $\late_\edge$ is continuous, non-decreasing functions, it is trivial that $\cost$ is convex.} we have
%
%\begin{equation}
% \cost \parens*{\frac{1}{\nRuns} \sum_{\run =\start}^{\nRuns} \flow^\run } - \cost \parens{\flowbase} \le   \frac{1}{\nRuns} \sum_{\run =\start}^{\nRuns} \bracks*{ \cost \parens{\flow^\run} - \cost \parens*{\flowbase}} \le \frac{ \nPairs \log \parens*{\nRoutes/\nPairs}}{  \nRuns} + \frac{  \nPairs \lips_0^2}{2}. \label{eq:ExpGrad_regret}
%\end{equation}

%Therefore, by choosing $  = \sqrt{\frac{\log\parens*{\nRoutes/\nPairs}}{\nRuns \lips_0^2}}$, from \eqref{eq:ExpGrad_regret}, we have:
%\begin{equation*}
%\cost \parens*{\flowave^{\nRuns} } - \cost \parens{\flowbase} \le \frac{3}{2} \frac{\nPairs \lips_0 \sqrt{\log \parens*{\nRoutes/\nPairs}}}{\sqrt{T}}  = \frac{3}{2} \frac{\nPairs \ratmax^2 \length \ub \sqrt{\log \parens*{\nRoutes/\nPairs}}}{\sqrt{T}}.
%\end{equation*}
%This concludes the proof.       









==> Conclusion.tex <==
\revise{To be filled in...}

==> Scraps/game_form_FOLC.tex <==





\subsection{Problem setup}
% \label{sec:prob_setup}
%
Consider a finite set of facilities $\edges = \braces{\edge(1), \edge(2), \ldots, \edge(\nEdges)}$ (we denote $\abs{\edges} = \nEdges$) and a set $\pairs$ of $\nPairs$ types of users. We denote by $\routes_\pair = \braces*{\route(\pair, \coord ), \forall \coord = 1,\ldots, \abs{\nRoutes}_{\pair}}  \subset \{0,1\}^\nEdges$ the set of strategies that $\pair$-type users have over the facilities. Intuitively, $\route(\pair, \coord )_{\edge} =1$ if and only if in the strategy $\route(\pair, \coord)$, $\pair$-type users select the facility $\edge$ (for any $\edge =1,\ldots, \nEdges$).  
 
Corresponding to each edge $\edge \in \edges$, there exists an \emph{edge-latency function} \mbox{$\late_{\edge}: \Rpos \rightarrow \Rpos$}. Throughout this work, we assume that $\late_{\edge}$ is non-negative, differentiable and non-decreasing. As the game proceeds, for each $\pair \in \pairs$, a certain amount of nonatomic traffic (called the $\pair$-type~traffic) will be sent from $\source_\pair$ to $\sink_\pair$ via the paths in $\routes_\pair$. If the total load of $\pair$-type traffic travelling edge $\edge$ is $\load_{\pair,\edge}$, then the latency cost on this edge is given by $\late_{\edge} \parens*{\sum_{\pair \in \pairs} \load_{\pair, \edge} }$. We denote the set of all edge-latency functions by $\Late= \braces*{\loss_\edge, \forall \edge \in \edges}$.

\begin{definition}
    Each tuple $\Gamma:= \parens*{\graph, \pairs, \bracks*{\graph_\pair}_{\pair \in \pairs}, \Loss}$ as described above defines a routing game~instance.    
\end{definition}





%------------------------------------------
%---------------------------------------
%
%
%
\subsection{Learning models}
%
%
Let $\rat_\pair$ denote the total rate of $\pair$-type traffic travelling from $\source_\pair$ to $\sink_\pair$; view it differently, $\rat_\pair$ can also be understood as the demand of traffic needed to be sent from $\source_\pair$ to $\sink_\pair$. When we want explicitly keep track of the traffic rates $\rat$, we denote the game by $\Gamma_{\rat}$ instead of $\Gamma$.



Throughout this work, we will make the following blanket~assumptions:
%often study the routing games under the following assumptions:

\begin{assumption}\label{assum:rate}
$\forall \pair\in\pairs$, $\rat_\pair$ is generated randomly from an unknown distribution on $\bracks{0,\ratmax}$ for some $\ratmax>0$.
%where \mbox{$0<\ratmax< + \infty$}.
\end{assumption}




These are very mild assumptions that are satisfied by most (if not all) applicable situations in practice \textendash\ including the widely used BPR (Bureau of Public Roads) model \mbox{$\late_{\edge}(x) = a_{\edge} + b_{\edge} x^{\pexp}$}.
Importantly, nonlinear BPR functions are not Lipschitz continuous over all of $\R_{+}$, but they are Lipschitz over the interval $[0,\nPairs\rat_{\max}]$ that indicates the maximum available traffic that can ever occur in the network.
For this reason, Assumption \ref{assum:latency} implies that each edge-congestion function $\late_{\edge}$ can be effectively assumed to be $\bderiv$-Lipschitz continuous for some $\bderiv>0$.
In the rest of our paper we will consider this to be the case without making further mention to it. 




Settings:


\begin{assumption} \label{assum:latency}
$\forall \edge \in \edges$, $\late_{\edge}$ is a nonnegative, nondecreasing and locally Lipschitz~continuous function.
%$\bderiv$-Lipschitz continuous.
%moreover, they are $\bderiv$-Lipschitz continuous on $\Rpos$, \ie there exists $\bderiv >0$ such that \mbox{$\late^{\prime}_{\edge} \parens{\real} \le \bderiv$}, \mbox{$\forall \real \in \Rpos$}.
\end{assumption}










%------------------------------------------
%---------------------------------------
\section{\ac{fol} with network structure}
%----------------------------------------
%---------------------------------------
%
%
%
%%%%%
%%%%%--------------------------
\subsection{Latency optimization in routing games}
%
Consider a directed graph $\graphall$ with the set of \emph{edges} $\edges$ and the set of \emph{vertices} $\vertices$; we denote $ \nVertices = \abs{\vertices}$ and $ \nEdges = \abs{\edges} $.\footnote{For the sake of simplicity, we assume that $\graph$ is a simple directed graph; however, note that our results in this work can also be extended to cases where $\graph$ is a~multi-graph.} In $\graph$, there exists a set of pre-determined \emph{origin-destination pairs} \mbox{$\pairs = \braces*{\braces{\source_1 \mhyphen \sink_1}, \ldots, \braces{\source_\nPairs \mhyphen \sink_\nPairs}}$} where for any $\pair$, there exists a directed acyclic graph (DAG) $\graph_\pair \parens*{\vertices_\pair, \edges_\pair}$ being a sub-graph of $\graph$ and having $\source_\pair, \sink_\pair$ as the source vertex and destination vertex respectively. In the remainder of this work, we simply write $\pair \in \pairs$ to refer to the pair $\source_\pair \mhyphen \sink_\pair$.
% Associated with each pair $\pair \in \pairs$, there exists a \ac{DAG}, namely $\graph_\pair \parens*{\vertices_\pair, \edges_\pair}$, which is a \emph{sub-graph} of $\graph$ (\ie $\vertices_\pair \subseteq \vertices$ and $\edges_\pair \subseteq \edges$) that has $\source_\pair$ as the origin vertex and $\sink_\pair$ as the destination vertex.
For each $\pair \in \pairs$, let $\routes_\pair$ denote the \emph{set of all (simple and directed) paths} in $\graph_\pair$ going from $\source_\pair$ to $\sink_\pair$.\footnote{Without loss of generality, for any $\pair \in \pairs$, we assume that for any vertex $\vertex \in \vertices_\pair$, there exists at least one path $\route \in \routes_\pair$ passing through $\vertex$.} We let $\routes = \bigcup_{\pair \in \pairs} \routes_\pair$ and define \mbox{$\nRoutes = \abs{\routes}$}.


Corresponding to each edge $\edge \in \edges$, there exists an \emph{edge-latency function} \mbox{$\late_{\edge}: \Rpos \rightarrow \Rpos$}. Throughout this work, we assume that $\late_{\edge}$ is non-negative, differentiable and non-decreasing. As the game proceeds, for each $\pair \in \pairs$, a certain amount of nonatomic traffic (called the $\pair$-type~traffic) will be sent from $\source_\pair$ to $\sink_\pair$ via the paths in $\routes_\pair$. If the total load of $\pair$-type traffic travelling edge $\edge$ is $\load_{\pair,\edge}$, then the latency cost on this edge is given by $\late_{\edge} \parens*{\sum_{\pair \in \pairs} \load_{\pair, \edge} }$. We denote the set of all edge-latency functions by $\Late= \braces*{\loss_\edge, \forall \edge \in \edges}$.

\begin{definition}
    Each tuple $\Gamma:= \parens*{\graph, \pairs, \bracks*{\graph_\pair}_{\pair \in \pairs}, \Loss}$ as described above defines a routing game~instance.    
\end{definition}















%%%%%%%%
%-----------------------------
\subsection{Equilibrium flow learning in routing games}





%%%%%%%%
%-----------------------------
\subsection{Weighted $m$-size subsets}







%------------------------------------------
%---------------------------------------
%
%
%
\section{Centralized vs distributed}
In this work, we focus on the distributed routing game that models network systems where the transmission of traffic is determined by decisions made by each vertex. Before formally defining the game, we introduce new notation: for any vertex $\vertex \in \vertices$, let $\Out_{\pair,\vertex}, \In_{\pair,\vertex} \subset \edges_\pair$ be the sets of outgoing edges and the set of incoming edges of vertex $\vertex$ in the sub-graph $\graph_\pair$; we also define $\pairs_{\vertex} = \braces*{ \pair \in \pairs: \vertex \in \vertices_{\pair}}$, \ie the set of all O-D pairs whose the corresponding sub-graph contains $\vertex$ and define $\Out_{\vertex} := \bigcup_{\pair \in \pairs} \Out_{\pair,\vertex}$. 


In the \emph{distributed routing game} with the network structure  $\parens*{\graph, \pairs, \bracks*{\graph_\pair}_{\pair \in \pairs}, \Loss}$, each vertex $\vertex \in \vertices$ needs to choose a \emph{distributed flow} vector $\dflow_{\vertex}= \parens{\dflow_{\vertex, \pair,\edge}}_{\pair \in \pairs_{\vertex}, \edge \in \Out_{\pair,\vertex}}$ where $\dflow_{\vertex,\pair, \edge}$ represents the proportion of $\pair$-type traffic arriving at $\vertex$ (if any) that is re-distributed to the outgoing edge $\edge \in \Out_{\pair,\vertex}$. The set of all feasible \emph{distributed flows} at vertex $\vertex$ is:
\begin{equation}
    \dflows_{\vertex} = \braces*{\dflow_{\vertex} \in [0,1]^{\abs{\Out_{\vertex}}}: \sum_{\edge \in \Out_{\pair,\vertex}} \dflow_{\vertex,\pair,\edge} = 1, \forall \pair \in \pairs_{\vertex}}
\end{equation}

For the sake of brevity, we also define $\dis \dflows = \bigtimes_{\vertex \in \vertices} \dflows_{\vertex}$ and often write $\dflow = (\dflow_{\vertex})_{\vertex \in \vertices} \in \dflows$ to refer to the vector concatenated from $\dflow_{\vertex} \in \dflows_{\vertex}$. In order to analyze the network when the traffic is distributed according to a distributed flows $\dflow_{\vertex}$ at $\vertex \in \vertices$, we introduce two new notation: let $\ar_{\pair, \vertex} (\dflow)$ denote the proportion of $\pair$-type (for $\pair \in \pairs_{\vertex}$) traffic arriving at vertex $\vertex$ and let $\nload_{\pair, \edge} (\dflow)$ denote the proportion of $\pair$-type traffic passing through an edge $\edge$ (for $\edge \in \edges_\pair$). These quantities satisfy the following conditions:
\begin{align}
     \ar_{\pair, \source_\pair} (\dflow) & = 1, \forall \pair \in \pairs, \label{eq:con_1}\\
    %
     \nload_{\pair, \edge} (\dflow) & = \dflow_{\vertex, \pair, \edge} \cdot \ar_{\pair, \vertex}(\dflow), \forall \vertex \in \vertices, \forall \pair \in \pairs_{\vertex}, \forall \edge \in \Out_{\pair, \vertex},  \label{eq:con_2}\\
    %
     \ar_{\pair, \vertexalt} & = \sum_{\edgealt \in \In_{\pair, \vertexalt}} \nload_{\pair, \vertexalt} (\dflow), \forall \vertexalt \in \vertices, \forall \pair \in \pairs_{\vertex} . \label{eq:con_3}
\end{align}
%
Intuitively, \eqref{eq:con_1} means that by default, for any pair $\pair \in \pairs$, all $\pair$-type traffic is initialized at the source vertex $\source_\pair$; \eqref{eq:con_2} comes from the definition of $\dflow_{\vertex, \pair, \edge}$: it is the proportion of $\pair$-type traffic arriving at vertex $\vertex$ (\ie $\ar_{\pair, \vertex}(\dflow)$) that is distributed on the edge $\edge$; finally, \eqref{eq:con_3} says that the amount of $\pair$-type traffic arriving at a vertex is the summation of all $\pair$-type traffic passing through all incoming edges (in $\graph_\pair$) of $\vertex$.











==> Scraps/introduction_FOLC.tex <==







In this work, we consider a general framework of \ac{fol}: consider a set of \emph{facilities} and a set of \emph{strategies} each of which represents a combination of facilities; at each epoch, the learner chooses a set of \emph{weights} to assign to the available strategies under pre-determined constraints; a cost depending on the overlapping weights on facilities and other parameters (that might be randomly generated in each epoch from an unknown distribution) occurs; finally, an estimation of gradients of the cost \wrt the chosen weights is observed. The learner's goal in \ac{fol} is to quickly find the fixed weights assignment that minimizes the aggregate costs. An illustrative example of \ac{fol} is the problem of traffic distribution in networks: the facilities correspond to the edges, the strategies correspond to the paths and the weights are the flows (\ie mass) of traffic that are distributed on the paths. \ac{fol} captures well-known network problems such as equilibrium flows learning in routing game and latency minimization \cite{roughgarden2007routing}. Beyond network applications, \ac{fol} also covers a wide range of previously studied sequential learning problems with combinatorial structure, \eg $m$-sized subsets, learning permutations, task assignments \citep{cesa2012}.


% \ac{fol} and its instances pose two main challenges: 
%
% \begin{itemize}
%     \item[] \emph{Challenge 1:} Due to its combinatorial structure, the dimension of decision variables (\ie the number of strategies) in \ac{fol} is often exponentially large. This raises a double-faceted challenge: algorithms running in \ac{fol} are scalable only if both the time complexity of each iteration and the dependence of speed of convergence are in logarithmic order of the dimension.
%     %
%     \item[] \emph{Challenge 2:} There are two main settings in \ac{fol}: \emph{stochastic regime}---where cost functions change stochastically between iterations and \emph{stationary regime}---where cost functions are fixed. 
% \end{itemize}


Due to its combinatorial structure, the dimension of decision variables in \ac{fol} (\ie the number of strategies) is often exponentially large. This raises a double-faceted challenge: algorithms running in \ac{fol} are scalable only if both the time complexity of each iteration and the speed of convergence are in logarithmic order of the dimension. On the other hand, depending on the applications, it is natural to consider \ac{fol} in different regimes, \eg stochastic regime where cost functions change stochastically between epochs or stationary regime where all parameters are fixed. Different instances of \ac{fol} also involve objective functions having different characteristics (\eg Lipschitz-continuity, smoothness). These regimes and variations allow different convergence guarantees. Current state-of-the-art algorithms have several common drawbacks:
\begin{enumerate*}[{\itshape (a)}]
    \item they might provide optimal guarantees in one regime but fails to do so in others;
    %
    \item it is required to tune these algorithms a priori based on parameters of latency functions (that are not always available);
    %
    \item there exists no explicit implementation of these algorithms in a distributed manner with an efficient running time.
\end{enumerate*}



\paragraph{Our contributions.}


In this work, we propose the \ac{fol} framework and show that many previously studied models fit into this framework. In the generic setting of \ac{fol}, our paper focuses on the following key question:
%
\begin{center}
    \begin{minipage}[c][2.1cm]{0.9\textwidth}
    \begin{center}
        \itshape
        Is it possible to design an adaptive learning algorithm that is \textbf{efficiently implementable} in a distributed manner while \textbf{simultaneously} obtain optimal convergence's guarantees in both the stochastic and stationary regimes?
    \end{center}
    \end{minipage} 
\end{center}

Our contributions are arranged into two groups as~follows:
%
%
\begin{enumerate}
[left=\parindent]
%
\item
First, we study the \emph{centralized routing game} which is a relaxed version where all vertices are allowed to \emph{freely} communicate with one another and have access to all information up to the current time-step; alternatively, it is equivalent to assume a centralized agent having total control over the network and deciding the load of traffic on each available paths/routes. While the classical version of exponential weights achieves an $\bigoh \parens*{(\log\nRoutes)/ \sqrt{\nRuns}}$ convergence rate in the stochastic regime (this is order optimal), it fails to achieve optimal guarantees in the stationary regime with smooth objective functions. We extend results from \cite{vu2021} (which are limited to equilibrium flow learning) and obtain the following results:
%
    \begin{enumerate}[(a) ]
        \item
        We present the \acdef{AcceEW} algorithm---a combination of the \acl{EW} algorithm and Nesterov's acceleration---implemented in the centralized routing game. We show that \ac{AcceEW} achieves an (order) optimal rate of convergence of $\bigoh((\log\nRoutes)/\nRuns^{2})$ in the stationary regime whenever the involved objective function is smooth (\eg when the latency functions are smooth in the congestion-cost optimization problem or when they are Lipschitz-continuous in the equilibrium flow learning problem). However, \ac{AcceEW} fails to converge in the stochastic regime.
        %
        \item
        We develop an \acdef{AEW} algorithm. \ac{AEW} \emph{simultaneously} achieves (order) optimal rates of convergence in all settings: in the stochastic case, it obtains a convergence rate $\bigoh(\log\nRoutes/\sqrt{\nRuns})$; in the stationary regime, this guarantee becomes $\bigoh((\log\nRoutes)/\sqrt{\nRuns})$ when the objective function is Lipschitz-continuous and $\bigoh((\log\nRoutes)/{\nRuns^2})$ when the objective function is smooth.
        Importantly, \ac{AEW} requires no prior tuning to obtain these convergence rates. 
    \end{enumerate}
%
%
%
\item Second, we extend the EW, \ac{AcceEW} and \ac{AEW} algorithms for learning in the distributed routing game where the vertices control local decisions and are only able to communicate with their direct neighbors. We show that our distributed variants of EW, \ac{AcceEW} and \ac{AEW} algorithms provide the following improvements:
 \begin{enumerate}[(a) ,start = 3]
        \item
        They are \emph{fully distributed}: in order to operate, each vertex only needs to have access to the local information (and a synchronous clock) without requiring knowledge of the topology of the whole network nor explicit coordination between vertices. 
        %
        \item 
        These distributed algorithms enjoy (order) \emph{optimal convergence rates} as in the centralized setting and retain all dependence of the convergence rates on the time horizon $\nRuns$ and the number of paths in the network $\nRoutes$. In particular, the distributed \ac{AEW} algorithm simultaneously achieves optimal convergence rates in all settings without any prior tuning.
         %
         \item 
         Unlike their centralized variants (whose running time is polynomial in $\nRoutes$ which is exponentially large), the distributed variants of all three algorithms are \emph{efficiently implementable}: their running time are polynomial in terms of the number of edges and vertices in the network. This feature improves the scalability and implementability of learning in routing games where previous implementations of state-of-the-art algorithms are very restricted due to the curse of~dimensionality.
         %
         \item 
         Finally, we conduct several numerical experiments to illustrate the improvements that \ac{AcceEW}, \ac{AEW} and their distributed variants offer. 
    \end{enumerate}
%



\end{enumerate}
% 
% The key to achieving adaptation between the stationary and stochastic regimes is an ``inverse-sum-of-squares'' step-size as in the widely used AdaGrad algorithm of \citet{duchi2011adaptive};
% the moniker \ac{AEW} has been chosen in reference to AdaGrad.
% However, it is important to note that AdaGrad lacks an acceleration mechanism, so it only achieves an $\bigoh(1/\nRuns)$ rate in the stationary setting \citep{levy2018online}.
% This interpolation was first achieved by the AcceleGrad algorithm of \citet{levy2018online}, but only for \emph{unconstrained} problems.
% The UnixGrad proposal of \citet{levy2018online} subsequently lifted the ``unconstrained'' restriction and achieved the desired adaptation in constrained problems, but under the requirement of a bounded Bregman diameter.
% This requirement is crucial for our purposes, because it rules out the \acl{EW} template (the simplex has infinite entropic diameter):
% as a result, the provided rate is polynomial in the number of paths in the network, and hence unsuitable for large network instances.
% We are not aware of another method in the literature achieving similar guarantees as \ac{AEW}.


















